Contextualization and Generalization in Entity and Relation Extraction

During the past decade, neural networks have become prominent in Natural Language Processing (NLP), notably for their capacity to learn relevant word representations from large unlabeled corpora. These word embeddings can then be transferred and finetuned for diverse end applications during a supervised training phase. More recently, in 2018, the transfer of entire pretrained Language Models and the preservation of their contextualization capacities enabled to reach unprecedented performance on virtually every NLP benchmark, sometimes even outperforming human baselines. However, as models reach such impressive scores, their comprehension abilities still appear as shallow, which reveal limitations of benchmarks to provide useful insights on their factors of performance and to accurately measure understanding capabilities. In this thesis, we study the behaviour of state-of-the-art models regarding generalization to facts unseen during training in two important Information Extraction tasks: Named Entity Recognition (NER) and Relation Extraction (RE). Indeed, traditional benchmarks present important lexical overlap between mentions and relations used for training and evaluating models, whereas the main interest of Information Extraction is to extract previously unknown information. We propose empirical studies to separate performance based on mention and relation overlap with the training set and find that pretrained Language Models are mainly beneficial to detect unseen mentions, in particular out-of-domain. While this makes them suited for real use cases, there is still a gap in performance between seen and unseen mentions that hurts generalization to new facts. In particular, even state-of-the-art ERE models rely on a shallow retention heuristic, basing their prediction more on arguments surface forms than context.

==> front_back_matter/dedication.tex <==
%*******************************************************
% Dedication
%*******************************************************
\thispagestyle{empty}
%\phantomsection 
\refstepcounter{dummy}
\pdfbookmark[1]{Dedication}{Dedication}

\vspace*{3cm}
\medskip
\medskip
\medskip
% \begin{center}
    À ma famille.  
% \end{center}


==> tables/03-ner/per_type.tex <==
\begin{table}[h!]
 \begin{adjustwidth*}{}{-.3\textwidth}
 \caption{Per type F1 scores of models trained on CoNLL03 in domain and out-of-domain (averaged over 5 runs).}
 \label{table:03:per_types}
 %  \resizebox{\textwidth}{!}{
 %  \resizebox{\columnwidth}{!}{
 %  \begin{tabularx}{@{}lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr@{}}

 \scriptsize
 \begin{tabularx}{1.3\textwidth}{@{}l@{\hspace{1em}}*{4}{Y}r*{4}{Y}r*{4}{Y}r*{4}{Y}rY@{}}
 \toprule
 %   & \multicolumn{5}{c}{All} & & \multicolumn{5}{c}{Exact Match} & & \multicolumn{5}{c}{Partial Match} & & \multicolumn{5}{c}{Unseen}\\
 %   & ALL & LOC & MISC & ORG & PER & & ALL & LOC & MISC & ORG & PER & & ALL & LOC & MISC & ORG & PER & & ALL & LOC & MISC & ORG & PER\\
   & \multicolumn{4}{c}{LOC} & & \multicolumn{4}{c}{MISC} & & \multicolumn{4}{c}{ORG} & & \multicolumn{4}{c}{PER} & & \multicolumn{1}{c}{ALL}\\
   \cmidrule{2-5} \cmidrule{7-10} \cmidrule{12-15} \cmidrule{17-20} \cmidrule{22-22}
 %   & Exact & Partial & New & All & & Exact & Partial & New & All & & Exact & Partial & New & All & & Exact & Partial & New & All & & \multicolumn{1}{c}{All}\\
   & EM & PM & New & All & & EM & PM & New & All & & EM & PM & New & All & & EM & PM & New & All & & \multicolumn{1}{c}{All}\\
   \midrule
   \textbf{CoNLL03}\\
     BiLSTM + ELMo           & 96.0 & 72.6 & 83.3 & 93.1 &
                                 & 94.3 & 58.9 & 53.9 & 81.8 &
                                 & 96.0 & 80.8 & 83.5 & 89.6 &
                                 & 98.9 & 98.7 & 94.6 & 97.0 &
                                 & \textbf{91.8}\\
          BiLSTM + ELMo[0]   & 95.9 & 66.8 & 81.8 & 92.6 &
                                 & 94.4 & 58.2 & 52.5 & 81.6 &
                                 & 95.8 & 75.5 & 80.6 & 87.7 &
                                 & 98.7 & 98.3 & 92.4 & 95.8 &
                                 & 90.7\\
          Map + ELMo         & 93.8 & 58.3 & 75.3 & 89.7 &
                                 & 90.4 & 49.2 & 43.4 & 76.7 &
                                 & 93.3 & 75.7 & 72.8 & 84.1 &
                                 & 98.5 & 98.3 & 91.7 & 95.5 &
                                 & 88.7\\
          Map + ELMo[0]      & 92.0 & 49.2 & 50.0 & 84.5 &
                                 & 90.8 & 48.5 & 40.5 & 76.6 &
                                 & 92.2 & 62.8 & 60.9 & 77.6 &
                                 & 96.5 & 95.2 & 85.2 & 91.1 &
                                 & 83.4\\

  \midrule
 %   & \multicolumn{5}{c}{All} & & \multicolumn{5}{c}{Exact Match} & & \multicolumn{5}{c}{Partial Match} & & \multicolumn{5}{c}{Unseen}\\
 %   & ALL & LOC & MISC & ORG & PER & & ALL & LOC & MISC & ORG & PER & & ALL & LOC & MISC & ORG & PER & & ALL & LOC & MISC & ORG & PER\\
 %   & \multicolumn{4}{c}{LOC} & & \multicolumn{4}{c}{MISC} & & \multicolumn{4}{c}{ORG} & & \multicolumn{4}{c}{PER}\\
 %   & Exact & Partial & Unseen & All & & Exact & Partial & Unseen & All & & Exact & Partial & Unseen & All & & Exact & Partial & Unseen & All\\

  \textbf{CoNLL03 $\rightarrow$ OntoNotes$^{\ast}$}\\
% \textbf{CoNLL03 $\rightarrow$ ON$^{\ast}$}\\

  BiLSTM + ELMo      & 94.9 & 63.0 & 77.7 & 88.5 &
                         & 94.6 & 56.5 & 37.8 & 78.8 &
                         & 92.8 & 80.8 & 74.5 & 80.5 &
                         & 91.9 & 84.5 & 75.6 & 82.2 &
                         & \textbf{83.4} \\
  BiLSTM  + ELMo[0]  & 94.6 & 60.8 & 72.7 & 87.1 &
                         & 94.0 & 57.9 & 30.0 & 75.0 &
                         & 91.0 & 75.5 & 63.2 & 73.7 &
                         & 89.9 & 84.0 & 74.9 & 81.3 &
                         & 80.5\\
  Map + ELMo         & 94.8 & 62.2 & 76.7 & 88.3 &
                         & 92.5 & 57.9 & 33.9 & 77.2 &
                         & 81.8 & 77.1 & 68.6 & 74.6 &
                         & 93.7 & 86.5 & 71.1 & 81.5 &
                         & 82.2\\
  Map + ELMo[0]      & 92.7 & 48.0 & 53.4 & 82.5 &
                         & 92.8 & 62.0 & 42.1 & 80.6 &
                         & 81.3 & 63.0 & 49.6 & 60.8 &
                         & 91.8 & 79.3 & 67.3 & 76.2 &
                         & 75.0\\
  \bottomrule
  \end{tabularx}
 %  }
\end{adjustwidth*}
 \end{table}


==> tables/03-ner/qualitative.tex <==
\renewcommand{\arraystretch}{1}

\begin{table}[h!]
 %  \begin{table}[h!]
 \begin{adjustwidth*}{-.2\textwidth}{-.4\textwidth}
%   \resizebox{\textwidth}{!}{
 %  \resizebox{\columnwidth}{!}{
 \caption{In-domain qualitative examples from CoNLL03 test set. Bold words are not present in the training vocabulary.}
 \label{table:03:quali-id}
 
 \scriptsize
 
   \begin{tabularx}{1.6\textwidth}{@{}ll@{}}
  \toprule
    1 & ... during a disturbance at a [\textbf{McDonald} 's]$_{new}^{ORG}$ fast-food restaurant .\\
      \midrule
     BiLSTM-CRF + ELMo & ... during a disturbance at a \textcolor{OliveGreen}{[McDonald 's]$^{ORG}$} fast-food restaurant .\\
     BiLSTM-CRF + ELMo[0] & ... during a disturbance at a \textcolor{OrangeRed}{[McDonald]$^{PER}$} 's fast-food restaurant .\\
     Map-CRF + ELMo &  ... during a disturbance at a \textcolor{OliveGreen}{[McDonald 's]$^{ORG}$} fast-food restaurant .\\
     Map-CRF + ELMo[0] & ... during a disturbance at a \textcolor{OrangeRed}{[McDonald]$^{PER}$} 's fast-food restaurant .\\
     
  \midrule
    2 & [Pace]$^{PER}_{new}$ \textbf{outdistanced} three senior finalists ... \\
      \midrule
     BiLSTM-CRF + ELMo & \textcolor{OliveGreen}{[Pace]$^{PER}$} outdistanced three senior finalists ... \\
     BiLSTM-CRF + ELMo[0] & \textcolor{OrangeRed}{Pace} outdistanced three senior finalists ... \\
     Map-CRF + ELMo & \textcolor{OliveGreen}{[Pace]$^{PER}$} outdistanced three senior finalists ... \\
     Map-CRF + ELMo[0] & \textcolor{OrangeRed}{[Pace]$^{ORG}$} outdistanced three senior finalists ... \\

 \midrule
    3 & The loss by [Philadelphia]$^{ORG}_{exact}$ allowed the \textbf{idle} [Green Bay \textbf{Packers}]$^{ORG}_{new}$ ( 10-3 ) ...\\
      \midrule
     % &[Pace]$^{new}_{PER}$ \textbf{outdistanced} three senior finalists -- [Virginia \textbf{Tech}]$^{new}_{ORG}$ defensive end [\textbf{Cornell} Brown]$^{partial}_{PER}$ , [Arizona State]$^{partial}_{ORG}$\\
     %   & offensive tackle [Juan \textbf{Roque}]$^{partial}_{PER}$ and degensive end [Jared \textbf{Tomich}]$^{partial}_{PER}$ of [Nebraska]$^{new}_{LOC}$ . \\

     BiLSTM-CRF + ELMo & The loss by \textcolor{OliveGreen}{[Philadelphia]$^{ORG}$} allowed the idle \textcolor{OliveGreen}{[Green Bay Packers]$^{ORG}$} ( 10-3 ) ...\\
     BiLSTM-CRF + ELMo[0] & The loss by \textcolor{OrangeRed}{[Philadelphia]$^{LOC}$} allowed the idle \textcolor{OliveGreen}{[Green Bay Packers]$^{ORG}$} ( 10-3 ) ...\\
     Map-CRF + ELMo  & The loss by \textcolor{OliveGreen}{[Philadelphia]$^{ORG}$} allowed the idle \textcolor{OliveGreen}{[Green Bay Packers]$^{ORG}$} ( 10-3 ) ...\\
     Map-CRF + ELMo[0]  & The loss by \textcolor{OrangeRed}{[Philadelphia]$^{LOC}$} allowed the idle \textcolor{OliveGreen}{[Green Bay Packers]$^{ORG}$} ( 10-3 ) ...\\


  \midrule
    4 & SOCCER - [\textbf{BLINKER]}$^{PER}_{new}$ BAN\textbf{ LIFTED} . \\
    \midrule
     BiLSTM-CRF + ELMo & SOCCER - \textcolor{OliveGreen}{[BLINKER]$^{PER}$} BAN LIFTED . \\
     BiLSTM-CRF + ELMo[0] & SOCCER - \textcolor{OliveGreen}{[BLINKER]$^{PER}$} BAN LIFTED . \\
     Map-CRF + ELMo & SOCCER - \textcolor{OrangeRed}{BLINKER} BAN LIFTED . \\
     Map-CRF + ELMo[0] & SOCCER - \textcolor{OrangeRed}{BLINKER} BAN LIFTED . \\

 \midrule
   5 & [VANCOUVER]$^{ORG}_{new}$ AT [SAN \textbf{ANTONIO}]$^{LOC}_{partial}$\\
  \midrule
     BiLSTM-CRF + ELMo  & \textcolor{OliveGreen}{[VANCOUVER]$^{ORG}$} AT \textcolor{OliveGreen}{[SAN ANTONIO]$^{LOC}$}\\
     BiLSTM-CRF + ELMo[0] & \textcolor{OliveGreen}{[VANCOUVER]$^{ORG}$} AT \textcolor{OliveGreen}{[SAN ANTONIO]$^{LOC}$}\\
     Map-CRF + ELMo & \textcolor{OrangeRed}{[VANCOUVER]$^{LOC}$} AT \textcolor{OliveGreen}{[SAN ANTONIO]$^{LOC}$}\\
     Map-CRF + ELMo[0] & \textcolor{OrangeRed}{[VANCOUVER]$^{LOC}$} AT \textcolor{OliveGreen}{[SAN ANTONIO]$^{LOC}$}\\

 \midrule
  6 & ... fled with her family to the [United States]$^{LOC}_{exact}$ after the [\textbf{Communists}]$^{MISC}_{new}$ came to power ...\\
  \midrule
  BiLSTM-CRF + ELMo &  ... fled with her family to the \textcolor{OliveGreen}{[United States]$^{LOC}$} after the \textcolor{OliveGreen}{[Communists]$^{MISC}$} came to power ...\\
  BiLSTM-CRF + ELMo[0] &  ... fled with her family to the \textcolor{OliveGreen}{[United States]$^{LOC}$} after the \textcolor{OliveGreen}{[Communists]$^{MISC}$} came to power ...\\
  Map-CRF + ELMo &  ... fled with her family to the \textcolor{OliveGreen}{[United States]$^{LOC}$} after the \textcolor{OrangeRed}{Communists} came to power ...\\
  Map-CRF + ELMo[0] &  ... fled with her family to the \textcolor{OliveGreen}{[United States]$^{LOC}$} after the \textcolor{OrangeRed}{Communists} came to power ...\\

  \midrule
  7 & SOCCER - [FIFA]$^{ORG}_{exact}$ BOSS [\textbf{HAVELANGE}]$^{PER}_{new}$ \textbf{STANDS} BY [\textbf{WEAH}]$^{PER}_{new}$ .\\
  \midrule
  BiLSTM-CRF + ELMo & SOCCER - \textcolor{OliveGreen}{[FIFA]$^{ORG}$} BOSS \textcolor{OliveGreen}{[HAVELANGE]$^{PER}$} STANDS BY \textcolor{OrangeRed}{[WEAH]$^{ORG}$} .\\
  BiLSTM-CRF + ELMo[0] & SOCCER - \textcolor{OliveGreen}{[FIFA]$^{ORG}$} BOSS \textcolor{OrangeRed}{HAVELANGE} STANDS BY \textcolor{OrangeRed}{[WEAH]$^{ORG}$} .\\
  Map-CRF + ELMo & SOCCER - \textcolor{OliveGreen}{[FIFA]$^{ORG}$} BOSS \textcolor{OrangeRed}{HAVELANGE} STANDS BY \textcolor{OrangeRed}{WEAH} .\\
  Map-CRF + ELMo[0] & SOCCER - \textcolor{OrangeRed}{[FIFA BOSS]$^{ORG}$} \textcolor{OrangeRed}{HAVELANGE} STANDS BY \textcolor{OrangeRed}{[WEAH]$^{ORG}$} .\\

   \midrule
   8 & So far this year [\textbf{Zywiec}]$^{ORG}_{new}$, whose full name is [\textbf{Zaklady Piwowarskie w Zywcu} SA]$^{ORG}_{partial}$ , has \textbf{netted} ...\\
   \midrule
  BiLSTM-CRF + ELMo &  So far this year \textcolor{OliveGreen}{[Zywiec]$^{ORG}$}, whose full name is \textcolor{OrangeRed}{[Zaklady Piwowarskie]$^{ORG}$ w [Zywcu SA]$^{ORG}$} , has netted ...\\
  BiLSTM-CRF + ELMo[0] &  So far this year \textcolor{OrangeRed}{[Zywiec]$^{PER}$}, whose full name is \textcolor{OrangeRed}{[Zaklady Piwowarskie]$^{PER}$ w [Zywcu SA]$^{ORG}$} , has netted ...\\
  Map-CRF + ELMo &  So far this year \textcolor{OrangeRed}{[Zywiec]$^{LOC}$}, whose full name is \textcolor{OrangeRed}{[Zaklady Piwowarskie]$^{ORG}$ w [Zywcu SA]$^{ORG}$} , has netted ...\\
  Map-CRF + ELMo[0] & So far this year \textcolor{OrangeRed}{[Zywiec]$^{LOC}$}, whose full name is \textcolor{OrangeRed}{[Zaklady Piwowarskie]$^{PER}$ w [Zywcu SA]$^{ORG}$} , has netted ...\\
  \bottomrule
  \end{tabularx}
  \end{adjustwidth*}
 \end{table}

 \begin{table}[h!]
 %  \begin{table}[h!]
 \begin{adjustwidth*}{-.2\textwidth}{-.4\textwidth}
%   \resizebox{\textwidth}{!}{
 %  \resizebox{\columnwidth}{!}{
 
 \caption{Out-of-domain qualitative examples from OntoNotes$^\ast$ test set. Bold words are not present in the training vocabulary.}
 \label{table:03:quali-ood}
 
 \scriptsize
  \begin{tabularx}{1.6\textwidth}{@{}ll@{}}
  \toprule
     9 & \textbf{Was} [Sixty \textbf{Minutes}]$^{ORG}_{new}$ unfair to [Bill Clinton]$^{PER}_{exact}$ in \textbf{airing} [Louis Freeh]$^{PER}_{exact}$ 's charges against him ?\\
      \midrule
     BiLSTM-CRF + ELMo & Was \textcolor{OliveGreen}{[Sixty Minutes]$^{ORG}$} unfair to \textcolor{OliveGreen}{[Bill Clinton]$^{PER}$} in airing \textcolor{OliveGreen}{[Louis Freeh]$^{PER}$} 's charges against him ?\\
     BiLSTM-CRF + ELMo[0]& Was \textcolor{OrangeRed}{Sixty Minutes} unfair to \textcolor{OliveGreen}{[Bill Clinton]$^{PER}$} in airing \textcolor{OliveGreen}{[Louis Freeh]$^{PER}$} 's charges against him ?\\
     Map-CRF + ELMo  & Was \textcolor{OliveGreen}{[Sixty Minutes]$^{ORG}$} unfair to \textcolor{OliveGreen}{[Bill Clinton]$^{PER}$} in airing \textcolor{OliveGreen}{[Louis Freeh]$^{PER}$} 's charges against him ?\\
     Map-CRF + ELMo[0] & Was \textcolor{OrangeRed}{Sixty Minutes} unfair to \textcolor{OliveGreen}{[Bill Clinton]$^{PER}$} in airing \textcolor{OliveGreen}{[Louis Freeh]$^{PER}$} 's charges against him ?\\
  \midrule
     10 & [\textbf{Renaissance}]$^{ORG}_{new}$ is keeping its money entirely in cash \textbf{equivalents} ...\\
      \midrule
     BiLSTM-CRF + ELMo & \textcolor{OliveGreen}{[Renaissance]$^{ORG}$} is keeping its money entirely in cash equivalents ...\\
     BiLSTM-CRF + ELMo[0] & \textcolor{OrangeRed}{[Renaissance]$^{MISC}$} is keeping its money entirely in cash equivalents ...\\
     Map-CRF + ELMo & \textcolor{OliveGreen}{[Renaissance]$^{ORG}$} is keeping its money entirely in cash equivalents ...\\
     Map-CRF + ELMo[0] & \textcolor{OrangeRed}{[Renaissance]$^{MISC}$} is keeping its money entirely in cash equivalents ...\\
     \midrule
     11 & Actor [\textbf{Drugewbo Unitich}]$^{PER}_{new}$ tells how the show began . \\
      \midrule
     BiLSTM-CRF + ELMo  & Actor \textcolor{OliveGreen}{[Drugewbo Unitich]$^{PER}$} tells how the show began . \\
     BiLSTM-CRF + ELMo[0]  & Actor \textcolor{OliveGreen}{[Drugewbo Unitich]$^{PER}$} tells how the show began . \\
     Map-CRF + ELMo  & Actor \textcolor{OrangeRed}{[Drugewbo Unitich]$^{ORG}$} tells how the show began . \\
     Map-CRF + ELMo[0] & Actor \textcolor{OrangeRed}{[Drugewbo Unitich]$^{ORG}$} tells how the show began . \\
     \midrule
     12 & [\textbf{Toledo} Ohio]$^{LOC}_{partial}$ is quiet this morning after a planned march by a self - styled nazi group sparked a riot yesterday .\\
      \midrule
     BiLSTM-CRF + ELMo & \textcolor{OliveGreen}{[Toledo Ohio]$^{LOC}$} is quiet this morning after a planned march by a self - styled nazi group sparked a riot yesterday .\\
     BiLSTM-CRF + ELMo[0] & \textcolor{OliveGreen}{[Toledo Ohio]$^{LOC}$} is quiet this morning after a planned march by a self - styled nazi group sparked a riot yesterday . \\
     Map-CRF + ELMo & \textcolor{OrangeRed}{[Toledo]$^{ORG}$ [Ohio]$^{LOC}$} is quiet this morning after a planned march by a self - styled nazi group sparked a riot yesterday .\\
     Map-CRF + ELMo[0] & \textcolor{OrangeRed}{[Toledo Ohio]$^{ORG}$} is quiet this morning after a planned march by a self - styled nazi group sparked a riot yesterday . \\
     \midrule

     13 & The [\textbf{Pouchen}]$^{LOC}_{new}$ shoe plant, [\textbf{Dongguan}]$^{LOC}_{new}$ 's largest, \textbf{employs} 100,000 . \\
      \midrule
     BiLSTM-CRF + ELMo & The \textcolor{OliveGreen}{[Pouchen]$^{LOC}$} shoe plant, \textcolor{OliveGreen}{[Dongguan]$^{LOC}$} 's largest, employs 100,000 .  \\
     BiLSTM-CRF + ELMo[0] & The \textcolor{OliveGreen}{[Pouchen]$^{LOC}$} shoe plant, \textcolor{OrangeRed}{[Dongguan]$^{ORG}$} 's largest, employs 100,000 .  \\
     Map-CRF + ELMo & The \textcolor{OrangeRed}{[Pouchen]$^{ORG}$} shoe plant, \textcolor{OliveGreen}{[Dongguan]$^{LOC}$} 's largest, employs 100,000 .  \\
     Map-CRF + ELMo[0] & The \textcolor{OrangeRed}{[Pouchen]$^{ORG}$} shoe plant, \textcolor{OrangeRed}{[Dongguan]$^{ORG}$} 's largest, employs 100,000 .  \\
     \midrule
     14 & ... because the [\textbf{Kuroshio}]$^{LOC}_{new}$ current passes close by , the waters offshore were rich fishing grounds .\\
      \midrule
     BiLSTM-CRF + ELMo & ... because the \textcolor{OliveGreen}{[Kuroshio]$^{LOC}$} current passes close by , the waters offshore were rich fishing grounds .\\
     BiLSTM-CRF + ELMo[0]& ... because the \textcolor{OrangeRed}{[Kuroshio]$^{MISC}$} current passes close by , the waters offshore were rich fishing grounds .\\
     Map-CRF + ELMo & ... because the \textcolor{OrangeRed}{[Kuroshio]$^{MISC}$} current passes close by , the waters offshore were rich fishing grounds .\\
     Map-CRF + ELMo[0] & ... because the \textcolor{OrangeRed}{[Kuroshio]$^{PER}$} current passes close by , the waters offshore were rich fishing grounds .\\
     \midrule
     15 & [\textbf{Linpien}]$^{LOC}_{new}$ residents see this as an important asset for \textbf{attracting} tourism .\\
      \midrule
     BiLSTM-CRF + ELMo & \textcolor{OliveGreen}{[Linpien]$^{LOC}_{new}$} residents see this as an important asset for attracting tourism .\\
     BiLSTM-CRF + ELMo[0]& \textcolor{OrangeRed}{[Linpien]$^{PER}$} residents see this as an important asset for attracting tourism .\\
     Map-CRF + ELMo & \textcolor{OrangeRed}{[Linpien]$^{ORG}$} residents see this as an important asset for attracting tourism .\\
     Map-CRF + ELMo[0] & \textcolor{OrangeRed}{[Linpien]$^{ORG}$} residents see this as an important asset for attracting tourism .\\
     \midrule
     16 & [\textbf{Bolar}]$^{ORG}_{new}$ has denied that it switched the brand - name product for its own in such testing .\\
      \midrule
     BiLSTM-CRF + ELMo & \textcolor{OliveGreen}{[Bolar]$^{ORG}$} has denied that it switched the brand - name product for its own in such testing .\\
     BiLSTM-CRF + ELMo[0]& \textcolor{OrangeRed}{[Bolar]$^{PER}$} has denied that it switched the brand - name product for its own in such testing .\\
     Map-CRF + ELMo & \textcolor{OrangeRed}{[Bolar]$^{PER}$} has denied that it switched the brand - name product for its own in such testing .\\
     Map-CRF + ELMo[0] & \textcolor{OrangeRed}{[Bolar]$^{PER}$} has denied that it switched the brand - name product for its own in such testing .\\
     \midrule
     17 & ... it was \textbf{foretold} that one day a \textbf{mighty} son of [\textbf{Saturn}]$^{PER}_{new}$ would in turn overthrow him , \\
      \midrule
     BiLSTM-CRF + ELMo & ... it was foretold that one day a mighty son of \textcolor{OliveGreen}{[Saturn]$^{PER}$} would in turn overthrow him , \\
     BiLSTM-CRF + ELMo[0] &... it was foretold that one day a mighty son of \textcolor{OrangeRed}{[Saturn]$^{LOC}$} would in turn overthrow him ,  \\
     Map-CRF + ELMo & ... it was foretold that one day a mighty son of \textcolor{OrangeRed}{[Saturn]$^{ORG}$} would in turn overthrow him , \\
     Map-CRF + ELMo[0] &... it was foretold that one day a mighty son of \textcolor{OrangeRed}{[Saturn]$^{LOC}$} would in turn overthrow him ,  \\
  \bottomrule


  \end{tabularx}
  \end{adjustwidth*}
 \end{table}
 % \end{table}
 \renewcommand{\arraystretch}{1.2}

==> tables/03-ner/qualitative_old.tex <==
\renewcommand{\arraystretch}{1}

\begin{table}[t]
 %  \begin{table}[h!]
 \begin{adjustwidth*}{-.2\textwidth}{-.4\textwidth}
%   \resizebox{\textwidth}{!}{
 %  \resizebox{\columnwidth}{!}{
 \caption{In-domain qualitative examples from CoNLL03 test set. Bold words are not present in the training vocabulary.}
 \label{table:03:quali-id}
 
 \scriptsize
 
   \begin{tabularx}{1.6\textwidth}{@{}lll@{}}
  \toprule
    1 & &... during a disturbance at a [\textbf{McDonald} 's]$_{new}^{ORG}$ fast-food restaurant .\\
      \midrule
     BiLSTM-CRF + ELMo & \cmark  &... during a disturbance at a [McDonald 's]$^{ORG}$ fast-food restaurant .\\
     BiLSTM-CRF + ELMo[0]& \xmark & ... during a disturbance at a [McDonald]$^{PER}$ 's fast-food restaurant .\\
     Map-CRF + ELMo & \cmark  & ... during a disturbance at a [McDonald 's]$^{ORG}$ fast-food restaurant .\\
     Map-CRF + ELMo[0] & \xmark & ... during a disturbance at a [McDonald]$^{PER}$ 's fast-food restaurant .\\
     
  \midrule
    2 & & [Pace]$^{PER}_{new}$ \textbf{outdistanced} three senior finalists ... \\
      \midrule
     BiLSTM-CRF + ELMo & \cmark & [Pace]$^{PER}$ outdistanced three senior finalists ... \\
     BiLSTM-CRF + ELMo[0] & \xmark & Pace outdistanced three senior finalists ... \\
     Map-CRF + ELMo & \cmark & [Pace]$^{PER}$ outdistanced three senior finalists ... \\
     Map-CRF + ELMo[0] & \xmark & [Pace]$^{ORG}$ outdistanced three senior finalists ... \\

 \midrule
    3 & & The loss by [Philadelphia]$^{ORG}_{exact}$ allowed the \textbf{idle} [Green Bay \textbf{Packers}]$^{ORG}_{new}$ ( 10-3 ) ...\\
      \midrule
     % &[Pace]$^{new}_{PER}$ \textbf{outdistanced} three senior finalists -- [Virginia \textbf{Tech}]$^{new}_{ORG}$ defensive end [\textbf{Cornell} Brown]$^{partial}_{PER}$ , [Arizona State]$^{partial}_{ORG}$\\
     %   & offensive tackle [Juan \textbf{Roque}]$^{partial}_{PER}$ and degensive end [Jared \textbf{Tomich}]$^{partial}_{PER}$ of [Nebraska]$^{new}_{LOC}$ . \\

     BiLSTM-CRF + ELMo & \cmark\cmark& The loss by [Philadelphia]$^{ORG}$ allowed the idle [Green Bay Packers]$^{ORG}$ ( 10-3 ) ...\\
     BiLSTM-CRF + ELMo[0] & \xmark\cmark& The loss by [Philadelphia]$^{LOC}$ allowed the idle [Green Bay Packers]$^{ORG}$ ( 10-3 ) ...\\
     Map-CRF + ELMo  & \cmark\cmark& The loss by [Philadelphia]$^{ORG}$ allowed the idle [Green Bay Packers]$^{ORG}$ ( 10-3 ) ...\\
     Map-CRF + ELMo[0]  & \xmark\cmark & The loss by [Philadelphia]$^{LOC}$ allowed the idle [Green Bay Packers]$^{ORG}$ ( 10-3 ) ...\\


  \midrule
    4 & & SOCCER - [\textbf{BLINKER]}$^{PER}_{new}$ BAN\textbf{ LIFTED} . \\
    \midrule
     BiLSTM-CRF + ELMo & \cmark & SOCCER - [BLINKER]$^{PER}$ BAN LIFTED . \\
     BiLSTM-CRF + ELMo[0] & \cmark & SOCCER - [BLINKER]$^{PER}$ BAN LIFTED . \\
     Map-CRF + ELMo & \xmark & SOCCER - BLINKER BAN LIFTED . \\
     Map-CRF + ELMo[0] & \xmark & SOCCER - BLINKER BAN LIFTED . \\

 \midrule
   5 & & [VANCOUVER]$^{ORG}_{new}$ AT [SAN \textbf{ANTONIO}]$^{LOC}_{partial}$\\
  \midrule
     BiLSTM-CRF + ELMo & \cmark\cmark & [VANCOUVER]$^{ORG}$ AT [SAN ANTONIO]$^{LOC}$\\
     BiLSTM-CRF + ELMo[0] & \cmark\cmark & [VANCOUVER]$^{ORG}$ AT [SAN ANTONIO]$^{LOC}$\\
     Map-CRF + ELMo & \xmark\cmark & [VANCOUVER]$^{LOC}$ AT [SAN ANTONIO]$^{LOC}$\\
     Map-CRF + ELMo[0] & \xmark\cmark & [VANCOUVER]$^{LOC}$ AT [SAN ANTONIO]$^{LOC}$\\

 \midrule
  6 & & ... fled with her family to the [United States]$^{LOC}_{exact}$ after the [\textbf{Communists}]$^{MISC}_{new}$ came to power ...\\
  \midrule
  BiLSTM-CRF + ELMo & \cmark \cmark & ... fled with her family to the [United States]$^{LOC}$ after the [Communists]$^{MISC}$ came to power ...\\
  BiLSTM-CRF + ELMo[0] & \cmark\cmark & ... fled with her family to the [United States]$^{LOC}$ after the [Communists]$^{MISC}$ came to power ...\\
  Map-CRF + ELMo & \cmark\xmark & ... fled with her family to the [United States]$^{LOC}$ after the Communists came to power ...\\
  Map-CRF + ELMo[0] & \cmark\xmark & ... fled with her family to the [United States]$^{LOC}$ after the Communists came to power ...\\

  \midrule
  7 & & SOCCER - [FIFA]$^{ORG}_{exact}$ BOSS [\textbf{HAVELANGE}]$^{PER}_{new}$ \textbf{STANDS} BY [\textbf{WEAH}]$^{PER}_{new}$ .\\
  \midrule
  BiLSTM-CRF + ELMo & \cmark\cmark\xmark & SOCCER - [FIFA]$^{ORG}$ BOSS [HAVELANGE]$^{PER}$ STANDS BY [WEAH]$^{ORG}$ .\\
  BiLSTM-CRF + ELMo[0] & \cmark\xmark\xmark & SOCCER - [FIFA]$^{ORG}$ BOSS HAVELANGE STANDS BY [WEAH]$^{ORG}$ .\\
  Map-CRF + ELMo & \cmark\xmark\xmark & SOCCER - [FIFA]$^{ORG}$ BOSS HAVELANGE STANDS BY WEAH .\\
  Map-CRF + ELMo[0] & \xmark\xmark\xmark & SOCCER - [FIFA BOSS]$^{ORG}$ HAVELANGE STANDS BY [WEAH]$^{ORG}$ .\\

   \midrule
   8 & & So far this year [\textbf{Zywiec}]$^{ORG}_{new}$, whose full name is [\textbf{Zaklady Piwowarskie w Zywcu} SA]$^{ORG}_{partial}$ , has \textbf{netted} ...\\
   \midrule
  BiLSTM-CRF + ELMo & \cmark\xmark &  So far this year [Zywiec]$^{ORG}$, whose full name is [Zaklady Piwowarskie]$^{ORG}$ w [Zywcu SA]$^{ORG}$ , has netted ...\\
  BiLSTM-CRF + ELMo[0] & \xmark\xmark &  So far this year [Zywiec]$^{PER}$, whose full name is [Zaklady Piwowarskie]$^{PER}$ w [Zywcu SA]$^{ORG}$ , has netted ...\\
  Map-CRF + ELMo & \xmark\xmark &  So far this year [Zywiec]$^{LOC}$, whose full name is [Zaklady Piwowarskie]$^{ORG}$ w [Zywcu SA]$^{ORG}$ , has netted ...\\
  Map-CRF + ELMo[0] & \xmark\xmark & So far this year [Zywiec]$^{LOC}$, whose full name is [Zaklady Piwowarskie]$^{PER}$ w [Zywcu SA]$^{ORG}$ , has netted ...\\
  \bottomrule


  \end{tabularx}
  \end{adjustwidth*}
 \end{table}
 % \end{table}

 \begin{table}[t]
 %  \begin{table}[h!]
 \begin{adjustwidth*}{-.2\textwidth}{-.4\textwidth}
%   \resizebox{\textwidth}{!}{
 %  \resizebox{\columnwidth}{!}{
 
 \caption{Out-of-domain qualitative examples from OntoNotes$^\ast$ test set. Bold words are not present in the training vocabulary.}
 \label{table:03:quali-ood}
 
 \scriptsize
  \begin{tabularx}{1.6\textwidth}{@{}lll@{}}
  \toprule
     9 & & \textbf{Was} [Sixty \textbf{Minutes}]$^{ORG}_{new}$ unfair to [Bill Clinton]$^{PER}_{exact}$ in \textbf{airing} [Louis Freeh]$^{PER}_{exact}$ 's charges against him ?\\
      \midrule
     BiLSTM-CRF + ELMo & \cmark\cmark\cmark & Was [Sixty Minutes]$^{ORG}$ unfair to [Bill Clinton]$^{PER}$ in airing [Louis Freeh]$^{PER}$ 's charges against him ?\\
     BiLSTM-CRF + ELMo[0]& \xmark\cmark\cmark & Was Sixty Minutes unfair to [Bill Clinton]$^{PER}$ in airing [Louis Freeh]$^{PER}$ 's charges against him ?\\
     Map-CRF + ELMo & \cmark\cmark\cmark  & Was [Sixty Minutes]$^{ORG}$ unfair to [Bill Clinton]$^{PER}$ in airing [Louis Freeh]$^{PER}$ 's charges against him ?\\
     Map-CRF + ELMo[0] & \xmark\cmark\cmark & Was Sixty Minutes unfair to [Bill Clinton]$^{PER}$ in airing [Louis Freeh]$^{PER}$ 's charges against him ?\\
  \midrule
     10 & & [\textbf{Renaissance}]$^{ORG}_{new}$ is keeping its money entirely in cash \textbf{equivalents} ...\\
      \midrule
     BiLSTM-CRF + ELMo & \cmark & [Renaissance]$^{ORG}$ is keeping its money entirely in cash equivalents ...\\
     BiLSTM-CRF + ELMo[0]& \xmark & [Renaissance]$^{MISC}$ is keeping its money entirely in cash equivalents ...\\
     Map-CRF + ELMo & \cmark  & [Renaissance]$^{ORG}$ is keeping its money entirely in cash equivalents ...\\
     Map-CRF + ELMo[0] & \xmark & [Renaissance]$^{MISC}$ is keeping its money entirely in cash equivalents ...\\
     \midrule
     11 & & Actor [\textbf{Drugewbo Unitich}]$^{PER}_{new}$ tells how the show began . \\
      \midrule
     BiLSTM-CRF + ELMo & \cmark & Actor [Drugewbo Unitich]$^{PER}$ tells how the show began . \\
     BiLSTM-CRF + ELMo[0]& \cmark & Actor [Drugewbo Unitich]$^{PER}$ tells how the show began . \\
     Map-CRF + ELMo & \xmark & Actor [Drugewbo Unitich]$^{ORG}$ tells how the show began . \\
     Map-CRF + ELMo[0] & \xmark& Actor [Drugewbo Unitich]$^{ORG}$ tells how the show began . \\
     \midrule
     12 & & [\textbf{Toledo} Ohio]$^{LOC}_{partial}$ is quiet this morning after a planned march by a self - styled nazi group sparked a riot yesterday .\\
      \midrule
     BiLSTM-CRF + ELMo & \cmark & [Toledo Ohio]$^{LOC}$ is quiet this morning after a planned march by a self - styled nazi group sparked a riot yesterday .\\
     BiLSTM-CRF + ELMo[0]& \cmark & [Toledo Ohio]$^{LOC}$ is quiet this morning after a planned march by a self - styled nazi group sparked a riot yesterday . \\
     Map-CRF + ELMo & \xmark & [Toledo]$^{ORG}$ [Ohio]$^{LOC}$ is quiet this morning after a planned march by a self - styled nazi group sparked a riot yesterday .\\
     Map-CRF + ELMo[0] & \xmark&[Toledo Ohio]$^{ORG}$ is quiet this morning after a planned march by a self - styled nazi group sparked a riot yesterday . \\
     \midrule

     13 & & The [\textbf{Pouchen}]$^{LOC}_{new}$ shoe plant, [\textbf{Dongguan}]$^{LOC}_{new}$ 's largest, \textbf{employs} 100,000 . \\
      \midrule
     BiLSTM-CRF + ELMo & \cmark\cmark & The [Pouchen]$^{LOC}$ shoe plant, [Dongguan]$^{LOC}$ 's largest, employs 100,000 .  \\
     BiLSTM-CRF + ELMo[0]& \cmark\xmark & The [Pouchen]$^{LOC}$ shoe plant, [Dongguan]$^{ORG}$ 's largest, employs 100,000 .  \\
     Map-CRF + ELMo & \xmark\cmark  & The [Pouchen]$^{ORG}$ shoe plant, [Dongguan]$^{LOC}$ 's largest, employs 100,000 .  \\
     Map-CRF + ELMo[0] & \xmark\xmark & The [Pouchen]$^{ORG}$ shoe plant, [Dongguan]$^{ORG}$ 's largest, employs 100,000 .  \\
     \midrule
     14 & & ... because the [\textbf{Kuroshio}]$^{LOC}_{new}$ current passes close by , the waters offshore were rich fishing grounds .\\
      \midrule
     BiLSTM-CRF + ELMo & \cmark & ... because the [Kuroshio]$^{LOC}$ current passes close by , the waters offshore were rich fishing grounds .\\
     BiLSTM-CRF + ELMo[0]& \xmark & ... because the [Kuroshio]$^{MISC}$ current passes close by , the waters offshore were rich fishing grounds .\\
     Map-CRF + ELMo & \xmark  & ... because the [Kuroshio]$^{MISC}$ current passes close by , the waters offshore were rich fishing grounds .\\
     Map-CRF + ELMo[0] & \xmark & ... because the [Kuroshio]$^{PER}$ current passes close by , the waters offshore were rich fishing grounds .\\
     \midrule
     15 & & [\textbf{Linpien}]$^{LOC}_{new}$ residents see this as an important asset for \textbf{attracting} tourism .\\
      \midrule
     BiLSTM-CRF + ELMo & \cmark & [Linpien]$^{LOC}_{new}$ residents see this as an important asset for attracting tourism .\\
     BiLSTM-CRF + ELMo[0]& \xmark & [Linpien]$^{PER}$ residents see this as an important asset for attracting tourism .\\
     Map-CRF + ELMo & \xmark  & [Linpien]$^{ORG}$ residents see this as an important asset for attracting tourism .\\
     Map-CRF + ELMo[0] & \xmark & [Linpien]$^{ORG}$ residents see this as an important asset for attracting tourism .\\
     \midrule
     16 & & [\textbf{Bolar}]$^{ORG}_{new}$ has denied that it switched the brand - name product for its own in such testing .\\
      \midrule
     BiLSTM-CRF + ELMo & \cmark & [Bolar]$^{ORG}$ has denied that it switched the brand - name product for its own in such testing .\\
     BiLSTM-CRF + ELMo[0]& \xmark & [Bolar]$^{PER}$ has denied that it switched the brand - name product for its own in such testing .\\
     Map-CRF + ELMo & \xmark  & [Bolar]$^{PER}$ has denied that it switched the brand - name product for its own in such testing .\\
     Map-CRF + ELMo[0] & \xmark & [Bolar]$^{PER}$ has denied that it switched the brand - name product for its own in such testing .\\
     \midrule
     17 & & ... it was \textbf{foretold} that one day a \textbf{mighty} son of [\textbf{Saturn}]$^{PER}_{new}$ would in turn overthrow him , \\
      \midrule
     BiLSTM-CRF + ELMo & \cmark & ... it was foretold that one day a mighty son of [Saturn]$^{PER}$ would in turn overthrow him , \\
     BiLSTM-CRF + ELMo[0]& \xmark &... it was foretold that one day a mighty son of [Saturn]$^{LOC}$ would in turn overthrow him ,  \\
     Map-CRF + ELMo & \xmark  & ... it was foretold that one day a mighty son of [Saturn]$^{ORG}$ would in turn overthrow him , \\
     Map-CRF + ELMo[0] & \xmark &... it was foretold that one day a mighty son of [Saturn]$^{LOC}$ would in turn overthrow him ,  \\
  \bottomrule


  \end{tabularx}
  \end{adjustwidth*}
 \end{table}
 % \end{table}
 \renewcommand{\arraystretch}{1.2}

==> tables/03-ner/supp_per_genre.tex <==

 \begin{table}[t]
     \begin{adjustwidth*}{}{-.3\textwidth}
 \caption{Per genre out-of-domain micro-F1 scores of the BiLSTM-CRF model trained on CoNLL03. Results are averaged over 5 runs.}
 \label{table:03:supplementary-genre}
 \centering
 \scriptsize
 \begin{tabularx}{1.3\textwidth}{@{}l@{\hspace{1em}}*{4}{Y}r*{4}{Y}r*{4}{Y}r@{}}
 \toprule
 %   & \multicolumn{5}{c}{All} & & \multicolumn{5}{c}{Exact Match} & & \multicolumn{5}{c}{Partial Match} & & \multicolumn{5}{c}{Unseen}\\
 %   & ALL & LOC & MISC & ORG & PER & & ALL & LOC & MISC & ORG & PER & & ALL & LOC & MISC & ORG & PER & & ALL & LOC & MISC & ORG & PER\\
   & \multicolumn{4}{c}{broadcast conversation} & & \multicolumn{4}{c}{broadcast news} & & \multicolumn{4}{c}{news wire}\\
   \cmidrule{2-5} \cmidrule{7-10} \cmidrule{12-15}
   & EM & PM & New & All &\hspace{1em} & EM & PM & New & All &\hspace{1em} & EM & PM & New & All\\
   \midrule
 BERT            & 96.7 & 81.5 & 77.8 & 87.2 &
                 & 95.2 & 81.2 & 76.5 & 88.4 &
                 & 95.0 & 83.9 & 74.0 & 84.7 \\

 ELMo            & 95.6 & 77.5 & 76.1 & 85.0 &
                 & 95.5 & 79.0 & 77.8 & 88.6 &
                 & 92.4 & 81.1 & 73.2 & 82.9 \\

 Flair           & 95.1 & 71.9 & 57.3 & 78.0 &
                 & 94.8 & 77.4 & 71.4 & 86.5 &
                 & 93.3 & 79.4 & 66.6 & 80.4 \\

 \cdashline{1-15}
 ELMo[0]         & 95.5 & 76.2 & 68.3 & 82.6 &
                 & 95.1 & 79.2 & 75.9 & 88.0 &
                 & 91.4 & 78.3 & 66.4 & 80.0 \\


 GloVe + char    & 94.8 & 75.8 & 61.5 & 80.4 &
                 & 95.1 & 75.6 & 71.6 & 86.3 &
                 & 92.5 & 75.2 & 61.2 & 78.0 \\

  \midrule
  & \multicolumn{4}{c}{magazine} & & \multicolumn{4}{c}{telephone conversation} & & \multicolumn{4}{c}{web text}\\
  \cmidrule{2-5} \cmidrule{7-10} \cmidrule{12-15}
   & EM & PM & New & All & & EM & PM & New & All & & EM & PM & New & All\\
  \midrule
   BERT          & 96.3 & 82.5 & 72.8 & 82.4 &
                 & 93.1 & 88.9 & 78.1 & 84.5 &
                 & 92.1 & 81.6 & 66.1 & 79.5 \\

  ELMo           & 97.7 & 71.3 & 68.7 & 78.1 &
                 & 91.1 & 86.5 & 79.3 & 84.0 &
                 & 92.5 & 82.4 & 66.2 & 79.9 \\

  Flair          & 96.8 & 67.4 & 55.7 & 71.1 &
                 & 89.9 & 74.7 & 66.4 & 73.5 &
                 & 91.2 & 77.2 & 51.4 & 72.1 \\

 \cdashline{1-15}

 ELMo[0]         & 97.3 & 67.1 & 60.6 & 73.4 &
                 & 90.0 & 85.9 & 71.2 & 79.2 &
                 & 91.2 & 75.1 & 59.7 & 75.1 \\

  GloVe + char   & 97.1 & 64.6 & 56.0 & 70.7 &
                 & 91.3 & 84.4 & 72.2 & 79.7 &
                 & 91.1 & 69.1 & 48.9 & 69.2 \\

  \bottomrule
  \end{tabularx}
         \end{adjustwidth*}
 \end{table}

==> tables/04.3-retex/ner_in_rel.tex <==

    \begin{table}[!h]
    \centering
    \small
    
    \begin{tabularx}{\textwidth}{@{}l*{3}{Y}r*{3}{Y}r*{3}{Y}c@{}}
    
    \toprule
     & \multicolumn{3}{c}{NER in REL} &  & \multicolumn{3}{c}{NER Out REL} & & \multicolumn{3}{c}{ALL} \\
    \cline{2-4} \cline{6-8} \cline{10-12} 
    & Seen & Unseen & All & & Seen & Unseen & All &  & Seen & Unseen & All &  \\
    
    \midrule
    & \multicolumn{12}{c}{\textbf{ACE05}} \\
    \midrule
    
heuristic & 91.0$_{\stddev{\phantom{0.0}}}$ & - & 74.4$_{\stddev{\phantom{0.0}}}$ &  & 85.8$_{\stddev{\phantom{0.0}}}$ & - & 70.6$_{\stddev{\phantom{0.0}}}$ &  & 87.7$_{\stddev{\phantom{0.0}}}$ & - & 71.9$_{\stddev{\phantom{0.0}}}$ & \\


spert_entities & 93.8$_{\stddev{0.3}}$ & 67.8$_{\stddev{1.0}}$ & 89.1$_{\stddev{0.3}}$ &  & 87.8$_{\stddev{0.2}}$ & 70.9$_{\stddev{1.1}}$ & 84.8$_{\stddev{0.3}}$ &  & 89.9$_{\stddev{0.2}}$ & 69.8$_{\stddev{1.0}}$ & 86.3$_{\stddev{0.3}}$ & \\

    spert & 93.8$_{\stddev{0.3}}$ & 67.8$_{\stddev{0.9}}$ & 89.1$_{\stddev{0.4}}$ &  & 88.3$_{\stddev{0.4}}$ & 70.0$_{\stddev{1.4}}$ & 85.0$_{\stddev{0.3}}$ &  & 90.3$_{\stddev{0.3}}$ & 69.2$_{\stddev{0.9}}$ & 86.5$_{\stddev{0.3}}$ & \\

tabto_bert & 93.9$_{\stddev{0.3}}$ & 78.2$_{\stddev{1.7}}$ & 91.0$_{\stddev{0.5}}$ &  & 88.7$_{\stddev{0.5}}$ & 78.0$_{\stddev{1.5}}$ & 86.8$_{\stddev{0.6}}$ &  & 90.6$_{\stddev{0.4}}$ & 78.1$_{\stddev{1.5}}$ & 88.3$_{\stddev{0.6}}$ & \\

pure & 94.5$_{\stddev{0.3}}$ & 76.1$_{\stddev{0.8}}$ & 91.1$_{\stddev{0.3}}$ &  & 89.6$_{\stddev{0.2}}$ & 76.3$_{\stddev{0.6}}$ & 87.2$_{\stddev{0.2}}$ &  & 91.4$_{\stddev{0.1}}$ & 76.2$_{\stddev{0.6}}$ & 88.6$_{\stddev{0.1}}$ & \\

    \midrule
     & \multicolumn{12}{c}{\textbf{CoNLL04}} \\
    \midrule
    spert & 98.1$_{\stddev{0.5}}$ & 88.3$_{\stddev{0.4}}$ & 93.3$_{\stddev{0.3}}$ &  & 92.2$_{\stddev{1.1}}$ & 70.2$_{\stddev{0.5}}$ & 80.3$_{\stddev{0.4}}$ &  & 96.1$_{\stddev{0.6}}$ & 81.3$_{\stddev{0.3}}$ & 88.7$_{\stddev{0.3}}$ & \\

tabto_bert & 97.5$_{\stddev{0.5}}$ & 90.4$_{\stddev{0.8}}$ & 94.1$_{\stddev{0.6}}$ &  & 91.1$_{\stddev{2.5}}$ & 72.0$_{\stddev{0.6}}$ & 80.7$_{\stddev{1.2}}$ &  & 95.4$_{\stddev{0.7}}$ & 83.3$_{\stddev{0.3}}$ & 89.3$_{\stddev{0.4}}$ & \\

pure_cased & 97.7$_{\stddev{0.6}}$ & 89.0$_{\stddev{0.5}}$ & 93.5$_{\stddev{0.4}}$ &  & 91.8$_{\stddev{0.3}}$ & 69.2$_{\stddev{1.4}}$ & 79.5$_{\stddev{0.8}}$ &  & 95.8$_{\stddev{0.4}}$ & 81.4$_{\stddev{0.7}}$ & 88.5$_{\stddev{0.5}}$ & \\

spert_entities & 98.3$_{\stddev{0.3}}$ & 89.0$_{\stddev{1.0}}$ & 93.9$_{\stddev{0.6}}$ &  & 92.7$_{\stddev{1.0}}$ & 71.4$_{\stddev{1.7}}$ & 81.1$_{\stddev{1.1}}$ &  & 96.5$_{\stddev{0.4}}$ & 82.2$_{\stddev{1.1}}$ & 89.3$_{\stddev{0.7}}$ & \\

heuristic & 99.4$_{\stddev{\phantom{0.0}}}$ & - & 51.4$_{\stddev{\phantom{0.0}}}$ &  & 98.9$_{\stddev{\phantom{0.0}}}$ & - & 45.2$_{\stddev{\phantom{0.0}}}$ &  & 99.3$_{\stddev{\phantom{0.0}}}$ & - & 49.2$_{\stddev{\phantom{0.0}}}$ & \\
    
    \midrule
    & \multicolumn{12}{c}{\textbf{SciERC}} \\
    \midrule
 
    spert-scibert & 82.8$_{\stddev{1.0}}$ & 65.2$_{\stddev{0.4}}$ & 69.5$_{\stddev{0.3}}$ &  & 72.5$_{\stddev{2.0}}$ & 57.1$_{\stddev{1.2}}$ & 61.2$_{\stddev{1.0}}$ &  & 80.3$_{\stddev{0.7}}$ & 63.4$_{\stddev{0.3}}$ & 67.6$_{\stddev{0.2}}$ & \\
    
    pure & 82.0$_{\stddev{1.2}}$ & 64.0$_{\stddev{1.0}}$ & 68.1$_{\stddev{1.0}}$ &  & 68.2$_{\stddev{2.4}}$ & 57.2$_{\stddev{0.8}}$ & 59.9$_{\stddev{0.9}}$ &  & 78.7$_{\stddev{1.0}}$ & 62.5$_{\stddev{0.9}}$ & 66.2$_{\stddev{0.9}}$ & \\
 
    spert_entities_scibert & 83.6$_{\stddev{0.5}}$ & 64.3$_{\stddev{1.2}}$ & 68.7$_{\stddev{1.0}}$ &  & 68.6$_{\stddev{3.1}}$ & 56.2$_{\stddev{1.6}}$ & 59.3$_{\stddev{1.7}}$ &  & 80.0$_{\stddev{1.0}}$ & 62.5$_{\stddev{1.0}}$ & 66.6$_{\stddev{0.9}}$ & \\
    
    heuristic & 92.6$_{\stddev{\phantom{0.0}}}$ & - & 21.0$_{\stddev{\phantom{0.0}}}$ &  & 92.6$_{\stddev{\phantom{0.0}}}$ & - & 23.2$_{\stddev{\phantom{0.0}}}$ &  & 92.6$_{\stddev{\phantom{0.0}}}$ & - & 21.5$_{\stddev{\phantom{0.0}}}$ & \\

    \bottomrule
    
    \end{tabularx}
    \caption{NER RECALL in or Out of Relation}
    \label{table:ner_in_rel}
    \end{table}


==> tables/04.3-retex/qk_bk.tex <==
\newcolumntype{C}[1]{>{\arraybackslash}p{#1}}

    \begin{table*}[h]
    
    \caption{Some qualitative examples of models' predictions on original (left column) and swapped (right) CoNLL04 sentences for the ``Kill'' relation. Despite a perfect Relation Extraction in the original sentences for all models, swapping head and tails results in several types of errors mainly regarding the direction of the relation. Predictions of incorrect original triples are in red. These examples are obtained from models trained with the same seed ($s=0$).}
    \label{table:qualitative_kill}
    
    % \small
    
    \begin{tabularx}{\textwidth}{@{}lYY@{}}
    
    \toprule
     \textbf{1} & \multicolumn{2}{C{0.8\textwidth}}{The Warren Commission determined that on Nov. 22 , 1963 , \textbf{A} fired a high-powered rifle at \textbf{B} 's motorcade from the sixth floor of what is now the Dallas County Administration Building , where he worked .} \\
    \midrule
      A, B &  Lee Harvey Oswald, Kennedy  & Kennedy, Lee Harvey Oswald\\
     \midrule
    Ent-SpERT & (A,B) & \textcolor{red}{(B,A)} \\
    SpERT & (A,B) & \textcolor{red}{(B,A)} \\
    TABTO & (A,B) & \textcolor{red}{(B,A)} \\
    PURE & (A,B) & \textcolor{red}{(B,A)} \\
    \midrule
    
    \midrule
     \textbf{2} & \multicolumn{2}{C{0.8\textwidth}}{Today 's Highlight in History : Twenty years ago , on June 6 , 1968 , at 1 : 44 a.m. local time , \textbf{B} died at Good Samaritan Hospital in Los Angeles , 25 -LCB- hours after he was shot at the Ambassador Hotel by \textbf{A} .} \\
    \midrule
     A, B &  Sirhan Bishara Sirhan, Sen. Robert F. Kennedy  &  Sen. Robert F. Kennedy, Sirhan Bishara Sirhan \\
     \midrule
     
    Ent-SpERT & (A,B) & \textcolor{red}{(B,A)} \\
    SpERT & (A,B) & \textcolor{red}{(B,A)} \\
    TABTO & (A,B) & \textcolor{red}{(B,A)} \\
    PURE & (A,B) & - \\
    \midrule
    
    \midrule
     \textbf{3} & \multicolumn{2}{C{0.8\textwidth}}{In 1968 , authorities announced the capture in London of \textbf{A} , suspected of the assassination of civil rights leader \textbf{B} .} \\
    \midrule
     A, B &  James Earl Ray, Dr. Martin Luther King Jr  & Dr. Martin Luther King Jr, James Earl Ray \\
     \midrule
     
    Ent-SpERT & (A,B) & (A,B) \textcolor{red}{(B,A)} \\
    SpERT & (A,B) & (A,B) \textcolor{red}{(B,A)} \\
    TABTO & (A,B) & (A,B) \\
    PURE & (A,B) & (A,B) \\
    \midrule
    
    \midrule
     \textbf{4} & \multicolumn{2}{C{0.8\textwidth}}{The Warren Commission determined that \textbf{A} fired at \textbf{B} from the sixth floor of what is now the Dallas County Administration Building .} \\
    \midrule
     A, B &  Oswald, Kennedy  & Kennedy, Oswald \\
     \midrule
     
    Ent-SpERT & (A,B) & - \\
    SpERT & (A,B) & (A,B) \textcolor{red}{(B,A)} \\
    TABTO & (A,B) & \textcolor{red}{(B,A)} \\
    PURE & (A,B) & (A,B) \\
    
    \bottomrule
    
    \end{tabularx}
    \end{table*}






==> tables/04.3-retex/ql_bk.tex <==
\newcolumntype{C}[1]{>{\arraybackslash}p{#1}}

    \begin{table*}[h]
    
    \caption{Some qualitative examples of models' predictions on original (left column) and swapped (right) CoNLL04 sentences for the ``Located in'' relation. This relation is often simply expressed by an apposition of the head and tail separated by a comma. Predictions of incorrect original triples are in red. These examples are obtained from models trained with the same seed ($s=0$).}
    
    \label{table:qualitative_loc}
    
    % \small
    
    \begin{tabularx}{\textwidth}{@{}lYY@{}}
    
    \toprule
     \textbf{1} & \multicolumn{2}{C{0.8\textwidth}}{
Reagan recalled that on the 40th anniversary of the Normandy landings he read a letter from a young woman whose late father had fought at \textbf{A} , a \textbf{B} sector .} \\
    \midrule
      A, B &  Omaha Beach, Normandy  & Normandy, Omaha Beach\\
    \midrule
    Ent-SpERT & (A,B) & - \\
    SpERT & (A,B) & - \\
    TABTO & (A,B) & - \\
    PURE & (A,B) & (A,B) \\
    \midrule
    
    \midrule
     \textbf{2} & \multicolumn{2}{C{0.8\textwidth}}{\textbf{A} , \textbf{B} ( AP )} \\
    \midrule
     A, B &  MILAN, Italy & Italy, MILAN \\
    \midrule
    
    Ent-SpERT & (A,B) & (A,B) \\
    SpERT & (A,B) & (A,B) \\
    TABTO & (A,B) & \textcolor{red}{(B,A)} \\
    PURE & (A,B) & - \\
    \midrule
    
    \midrule
    \textbf{3} & \multicolumn{2}{C{0.8\textwidth}}{In \textbf{A} , downed tree limbs interrupted power in parts of \textbf{B} .} \\
    \midrule
     A, B &  Indianapolis, Indiana & Indiana, Indianapolis \\
    \midrule
    
    Ent-SpERT & (A,B) & \textcolor{red}{(B,A)} \\
    SpERT & (A,B) & \textcolor{red}{(B,A)} \\
    TABTO & (A,B) & \textcolor{red}{(B,A)} \\
    PURE & (A,B) & \textcolor{red}{(B,A)} \\
    \midrule
    
    \midrule
    \textbf{4} & \multicolumn{2}{C{0.8\textwidth}}{The plane , owned by Bradley First Air , of \textbf{A} , \textbf{B} , was carrying cargo to Montreal for Emery Air Freight Corp. , an air freight courier service with a hub at the Dayton airport .} \\
    \midrule
     A, B &  Ottawa, Canada & Canada, Ottawa \\
    \midrule
    
    Ent-SpERT & (A,B) (Dayton airport, Canada) & (Dayton airport, Ottawa) \\
    SpERT & (A,B) (Dayton airport, Canada) & - \\
    TABTO & (A,B) & (A,B) \\
    PURE & (A,B) & (A,B) \\
    
    \bottomrule
    
    \end{tabularx}
    
    \end{table*}






==> tables/04.3-retex/swap.tex <==

    \begin{table}[!h]
    \centering
    \small
  
    \begin{tabularx}{\textwidth}{@{}ll*{2}{Y}r*{2}{Y}r*{2}{Y}c@{}}
    
    \toprule
    
     & & \multicolumn{2}{c}{NER} &  & \multicolumn{2}{c}{RE Boundaries} & & \multicolumn{2}{c}{RE Strict} \\
      
     \cline{3-4} \cline{6-7} \cline{9-10}
     & & Normal & Swap & & Normal & Swap & & Normal & Swap\\
     \midrule
     
    \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Kill}}} 
    
    & spert & 91.4$_{\stddev{1.2}}$ & 92.6$_{\stddev{1.2}}$ & 
            & 86.2$_{\stddev{1.4}}$ & 35.0$_{\stddev{5.6}}$ & 
            & 86.2$_{\stddev{1.4}}$ & 35.0$_{\stddev{5.6}}$  \\
            
    & spert_entities  & 91.6$_{\stddev{0.4}}$ & 91.7$_{\stddev{0.7}}$ &  
                    & 85.1$_{\stddev{0.9}}$ & 35.4$_{\stddev{6.5}}$ &
                    & 85.1$_{\stddev{0.9}}$ & 35.4$_{\stddev{6.5}}$ & \\
    
    & tabto_bert     & 92.0$_{\stddev{0.4}}$ & 92.8$_{\stddev{0.7}}$ &  
                    & 89.6$_{\stddev{1.3}}$ & 27.6$_{\stddev{3.8}}$ &  
                    & 89.6$_{\stddev{1.3}}$ & 27.6$_{\stddev{3.8}}$ &\\
                    
    & pure_cased    & 90.5$_{\stddev{0.6}}$ & 90.7$_{\stddev{0.5}}$ & 
                    & 84.1$_{\stddev{1.2}}$ & 52.3$_{\stddev{6.5}}$ & 
                    & 84.1$_{\stddev{1.2}}$ & 52.3$_{\stddev{6.5}}$ & \\
    
    \midrule
    
    \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Located}}} 
    & spert & 88.6$_{\stddev{1.1}}$ & 87.7$_{\stddev{1.1}}$ & 
            & 75.5$_{\stddev{1.4}}$ & 24.9$_{\stddev{9.2}}$ & 
            & 75.0$_{\stddev{2.0}}$ & 24.9$_{\stddev{9.2}}$\\
            
    & spert_entities  & 90.0$_{\stddev{0.7}}$ & 87.0$_{\stddev{2.1}}$ & 
                    & 78.3$_{\stddev{2.4}}$ & 30.3$_{\stddev{4.6}}$ &  
                    & 78.3$_{\stddev{2.4}}$ & 30.3$_{\stddev{4.6}}$ &    \\
    
    & tabto_bert    & 90.1$_{\stddev{1.5}}$ & 88.9$_{\stddev{0.8}}$ &
                    & 85.3$_{\stddev{3.9}}$ & 36.8$_{\stddev{6.3}}$ &  
                    & 85.3$_{\stddev{3.9}}$ & 36.1$_{\stddev{5.8}}$ &    \\
                    
    & pure_cased    & 89.0$_{\stddev{1.0}}$ & 83.7$_{\stddev{0.5}}$ &  
                    & 81.2$_{\stddev{2.6}}$ & 59.3$_{\stddev{3.0}}$ &  
                    & 81.2$_{\stddev{2.6}}$ & 59.3$_{\stddev{3.0}}$ &\\
        
    \bottomrule
    
    \end{tabularx}
    \caption{Swap}
    \label{table:swap}
    \end{table}


==> tables/04.3-retex/swap_prf.tex <==

    \begin{table}[!h]
    \centering
    \small
    
    \begin{tabularx}{\textwidth}{@{}lll*{3}{Y}r*{3}{Y}c@{}}
    
    \toprule
     
     & & & \multicolumn{3}{c}{NER} &  & \multicolumn{3}{c}{RE Strict} \\
      
     \cline{4-6} \cline{8-10}
     & & & P & R & F1 & & P & R & F1 \\
     \midrule
     
    \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{Kill}}} 
    & \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Normal}}} & spert & 91.7$_{\stddev{2.1}}$ & 91.0$_{\stddev{1.0}}$ & 91.4$_{\stddev{1.2}}$ &  & 88.1$_{\stddev{3.1}}$ & 84.4$_{\stddev{1.4}}$ & 86.2$_{\stddev{1.4}}$ & \\
    
    & & spert_entities & 91.7$_{\stddev{0.4}}$ & 91.5$_{\stddev{0.7}}$ & 91.6$_{\stddev{0.4}}$ &  & 82.9$_{\stddev{2.7}}$ & 87.6$_{\stddev{1.8}}$ & 85.1$_{\stddev{0.9}}$ & \\
    
    & & tabto_bert & 91.8$_{\stddev{0.6}}$ & 92.2$_{\stddev{0.5}}$ & 92.0$_{\stddev{0.4}}$ &  & 88.8$_{\stddev{1.6}}$ & 90.7$_{\stddev{3.3}}$ & 89.6$_{\stddev{1.3}}$ & \\
    
    & & pure_cased & 91.5$_{\stddev{0.9}}$ & 89.6$_{\stddev{0.6}}$ & 90.5$_{\stddev{0.6}}$ &  & 87.2$_{\stddev{2.1}}$ & 81.3$_{\stddev{1.1}}$ & 84.1$_{\stddev{1.2}}$ & \\
    
    \cline{2-10}
    %SWAP
    & \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Swap}}} & spert & 92.6$_{\stddev{1.8}}$ & 92.6$_{\stddev{0.8}}$ & 92.6$_{\stddev{1.2}}$ &  & 33.0$_{\stddev{4.4}}$ & 37.3$_{\stddev{7.4}}$ & 35.0$_{\stddev{5.6}}$ & \\

    & & spert_entities & 91.3$_{\stddev{0.9}}$ & 92.1$_{\stddev{0.7}}$ & 91.7$_{\stddev{0.7}}$ &  & 31.8$_{\stddev{5.3}}$ & 40.0$_{\stddev{8.3}}$ & 35.4$_{\stddev{6.5}}$ & \\
    
    & & tabto_bert & 92.8$_{\stddev{0.8}}$ & 92.7$_{\stddev{0.9}}$ & 92.8$_{\stddev{0.7}}$ &  & 26.8$_{\stddev{3.6}}$ & 28.4$_{\stddev{4.1}}$ & 27.6$_{\stddev{3.8}}$ & \\
    
    & & pure_cased & 92.0$_{\stddev{0.5}}$ & 89.5$_{\stddev{1.0}}$ & 90.7$_{\stddev{0.5}}$ &  & 65.2$_{\stddev{6.0}}$ & 44.0$_{\stddev{7.4}}$ & 52.3$_{\stddev{6.5}}$ & \\
    
    
    
    
    \midrule
    
    \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{Located in}}} 
    & \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Normal}}} 
    &spert & 89.8$_{\stddev{1.2}}$ & 87.5$_{\stddev{1.5}}$ & 88.6$_{\stddev{1.1}}$ &  & 77.2$_{\stddev{2.8}}$ & 73.0$_{\stddev{3.0}}$ & 75.0$_{\stddev{2.0}}$ & \\

    & & spert_entities & 90.1$_{\stddev{0.8}}$ & 89.8$_{\stddev{1.5}}$ & 90.0$_{\stddev{0.7}}$ &  & 80.8$_{\stddev{3.7}}$ & 76.2$_{\stddev{3.2}}$ & 78.3$_{\stddev{2.4}}$ & \\
    
    & & tabto_bert & 90.1$_{\stddev{1.3}}$ & 90.0$_{\stddev{1.8}}$ & 90.1$_{\stddev{1.5}}$ &  & 93.0$_{\stddev{3.3}}$ & 78.9$_{\stddev{4.6}}$ & 85.3$_{\stddev{3.9}}$ & \\
    
    & & pure_cased & 88.6$_{\stddev{1.1}}$ & 89.4$_{\stddev{1.8}}$ & 89.0$_{\stddev{1.0}}$ &  & 89.3$_{\stddev{4.0}}$ & 74.6$_{\stddev{3.7}}$ & 81.2$_{\stddev{2.6}}$ & \\
    
    \cline{2-10}
    %SWAP
    & \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Swap}}} 
    & spert & 87.3$_{\stddev{1.4}}$ & 88.0$_{\stddev{0.9}}$ & 87.7$_{\stddev{1.1}}$ &  & 34.8$_{\stddev{14.8}}$ & 19.5$_{\stddev{6.7}}$ & 24.9$_{\stddev{9.2}}$ & \\

    & & spert_entities & 86.7$_{\stddev{1.9}}$ & 87.4$_{\stddev{2.7}}$ & 87.0$_{\stddev{2.1}}$ &  & 38.0$_{\stddev{8.5}}$ & 25.4$_{\stddev{2.8}}$ & 30.3$_{\stddev{4.6}}$ & \\
    
    & & tabto_bert & 89.0$_{\stddev{0.6}}$ & 88.8$_{\stddev{0.9}}$ & 88.9$_{\stddev{0.8}}$ &  & 46.5$_{\stddev{6.6}}$ & 29.7$_{\stddev{5.7}}$ & 36.1$_{\stddev{5.8}}$ & \\
    
    & & pure_cased & 82.7$_{\stddev{0.8}}$ & 84.6$_{\stddev{0.8}}$ & 83.7$_{\stddev{0.5}}$ &  & 74.9$_{\stddev{7.6}}$ & 49.7$_{\stddev{4.7}}$ & 59.3$_{\stddev{3.0}}$ & \\
    
    \bottomrule
    
    \end{tabularx}
    \caption{Swap}
    \label{table:swap_prf}
    \end{table}


==> tables/04.3-retex/swap_prf_rev_no_loc.tex <==

    \begin{table*}[h]
    \centering
    \small
    
    \begin{tabularx}{\textwidth}{@{}lll*{3}{Y}r*{3}{Y}r*{3}{Y}c@{}}
    
    \toprule
     
     
     & & & \multicolumn{3}{c}{NER \uparrow} &  & \multicolumn{3}{c}{RE Strict \uparrow} &  & \multicolumn{3}{c}{Reverse RE Strict \downarrow} \\
      
     \cline{4-6} \cline{8-10} \cline{12-14}
     & & & P & R & F1 & & P & R & F1 & & P & R & F \\
     \midrule
     
    \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{Kill}}} 
    & \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Original}}} 
    
    
    & Ent-SpERT & 91.7$_{\stddev{0.4}}$ & 91.5$_{\stddev{0.7}}$ & 91.6$_{\stddev{0.4}}$ &  & 82.9$_{\stddev{2.7}}$ & 87.6$_{\stddev{1.8}}$ & 85.1$_{\stddev{0.9}}$ &  & - & - & - & \\
    
    & & SpERT & 91.7$_{\stddev{2.1}}$ & 91.0$_{\stddev{1.0}}$ & 91.4$_{\stddev{1.2}}$ &  & 88.1$_{\stddev{3.1}}$ & 84.4$_{\stddev{1.4}}$ & 86.2$_{\stddev{1.4}}$ &  & - & - & - & \\

    
    & & TABTO & 91.8$_{\stddev{0.6}}$ & 92.2$_{\stddev{0.5}}$ & \textbf{92.0}$_{\stddev{0.4}}$ &  & 88.8$_{\stddev{1.6}}$ & 90.7$_{\stddev{3.3}}$ & \textbf{89.6}$_{\stddev{1.3}}$ &  & - & - & - & \\
    
    & & PURE & 91.5$_{\stddev{0.9}}$ & 89.6$_{\stddev{0.6}}$ & 90.5$_{\stddev{0.6}}$ &  & 87.2$_{\stddev{2.1}}$ & 81.3$_{\stddev{1.1}}$ & 84.1$_{\stddev{1.2}}$ &  & - & - & - & \\
    
    \cline{2-14}
    %SWAP
    & \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Swap}}} 
    
    & Ent-SpERT & 91.3$_{\stddev{0.9}}$ & 92.1$_{\stddev{0.7}}$ & 91.7$_{\stddev{0.7}}$ &  & 31.8$_{\stddev{5.3}}$ & 40.0$_{\stddev{8.3}}$ & 35.4$_{\stddev{6.5}}$ &  & 52.8$_{\stddev{5.6}}$ & 65.8$_{\stddev{7.2}}$ & 58.5$_{\stddev{5.7}}$ & \\
    
    & & SpERT & 92.6$_{\stddev{1.8}}$ & 92.6$_{\stddev{0.8}}$ & \textbf{92.6}$_{\stddev{1.2}}$ &  & 33.0$_{\stddev{4.4}}$ & 37.3$_{\stddev{7.4}}$ & 35.0$_{\stddev{5.6}}$ &  & 54.8$_{\stddev{5.1}}$ & 61.3$_{\stddev{4.1}}$ & 57.8$_{\stddev{4.0}}$ & \\

    & & TABTO & 92.8$_{\stddev{0.8}}$ & 92.7$_{\stddev{0.9}}$ & \textbf{92.8}$_{\stddev{0.7}}$ &  & 26.8$_{\stddev{3.6}}$ & 28.4$_{\stddev{4.1}}$ & 27.6$_{\stddev{3.8}}$ &  & 57.8$_{\stddev{3.1}}$ & 61.3$_{\stddev{3.0}}$ & 59.5$_{\stddev{2.8}}$ & \\
    
    & & PURE & 92.0$_{\stddev{0.5}}$ & 89.5$_{\stddev{1.0}}$ & 90.7$_{\stddev{0.5}}$ &  & 65.2$_{\stddev{6.0}}$ & 44.0$_{\stddev{7.4}}$ & \textbf{52.3}$_{\stddev{6.5}}$ &  & 17.8$_{\stddev{2.3}}$ & 12.0$_{\stddev{2.3}}$ & \textbf{14.3}$_{\stddev{2.2}}$ & \\
    
    
    \bottomrule
    
    \end{tabularx}
    \caption{Detailed results of the Swap Relation Experiment with Precision, Recall and F1 scores.}
    \label{table:swap_prf_rev}
    \end{table*}


==> tables/04.3-retex/swap_rev_no_loc.tex <==

    \begin{table}[t]
    \centering
    \small
    
    \begin{tabularx}{\columnwidth}{@{}l*{2}{Y}r*{2}{Y}r*{2}{Y}c@{}}
    
    \toprule
     
    \multicolumn{1}{c}{\multirow{2}{*}{F1}} & \multicolumn{2}{c}{NER \uparrow} &  & \multicolumn{2}{c}{RE \uparrow} & & \multicolumn{2}{c}{revRE \downarrow} \\
      
     \cline{2-3} \cline{5-6} \cline{8-9}
    %  \cline{3-4} \cline{6-7} \cline{9-10}
     & O & S & & O & S & & O & S &\\
    \midrule
     
    Ent-SpERT & 91.6 & 91.7 &  & 85.1 & 35.4 &  & - & 58.5 & \\

    SpERT & 91.4 & \textbf{92.6} &  & 86.2 & 35.0 &  & - & 57.8 & \\
    
    TABTO & \textbf{92.0} & \textbf{92.8} &  & \textbf{89.6} & 27.6 &  & - & 59.5 & \\
    
    PURE & 90.5 & 90.7 &  & 84.1 & \textbf{52.3} &  & - & \textbf{14.3} & \\

    \bottomrule
    
    \end{tabularx}
    \caption{Performance on CoNLL04 test set sentences containing exactly one ``Kill'' relation in its original form (O) and where the relation head and tail are swapped (S). NER F1 score is micro-averaged while strict RE score only takes these relations into account. The revRE score corresponds to unwanted extraction of the reverse relation, symptomatic of the retention effect in the swapped setting.}
    \label{table:swap_rev}
    \end{table}


==> template/CHANGES <==
Changes in version 4.2 (September 2015)
o Fixed issue between titlesec and tocloft regarding
  part numbering in the ToC (classicthesis.sty). 
	Thanks to Enrico Gregorio and Henri Menke.
o Fixed bug with colored lines and graffiti 
  (classicthesis.sty). Thanks to Enrico Gregorio and
  Stefano Bragaglia for the fix! (Also switched
  graffiti from \slshape to \itshape.)
o Changed \vspace*{8ex} to \vspace{8ex} (Contents.tex)	
o Moved \cleardoublepage from end of Contents.tex 
  to appropriate position in ClassicThesis.tex
o \bflabel of acronym package removed, as it was 
  removed from acronym package and caused errors.
  Now set \aclabelfont to \acsfont for consistency.
o Converted major files to UTF-8 (thanks to Jörn Hees)
  (Bibliography.bib excluded for now as BibTeX cannot
  handle UTF-8)
o Added support for BibLaTeX in 
  classicthesis-config.tex and Bibliography.tex
	(thanks to Jörn Hees).
	For LyX we will have a work-around for testing.
o Added an example for one's own publication list
  (via BibLaTeX) in Publications.tex (renamed from 
	Publication.tex)
o Replaced/updated scrpage2 with scrlayer-scrpage 
  in classicthesis.sty (thanks to Ivo Pletìkosić).
X Worked on Appendix case with floatperchapter 
  (works for captions but not for references so far)
	Thanks to Claus Lahiri and Clemens Niederberger 
	for their help on this.
	[REMOVED DUE TO OTHER PROBLEMS, SEE ISSUE #82]	
X Removed fixltx2e from classicthesis-config.tex and
  have classicthesis.sty use or emulate the latest 
	LaTeX kernel via latexrelease (option: latest)
  (thanks to Jörn Hees).
	[REMOVED AS IT IS NOT AVAILABLE IN MANY 
	DISTRIBUTIONS, SEE ISSUE #107]
	
Changes in version 4.1 (August 2012)
o Working towards XeLaTeX support:
	- "ifxetex" package for checking whether
	  XeTeX is in use (classicthesis.sty)
	- Adjusted part, chapter, and tocEntry 
	- Thanks to Joerg Weber for his ideas and code
	- Option "pdfspacing" does not work for XeTeX
	  and is disabled when XeTeX is running
	  (maybe implement spacing with fontspec later)
o Load additional packages in order to 
  reduce warnings (classicthesis-config.tex)
	- "textcomp" to fix warnings with missing font 
	  shapes
	- "scrhack" to fix warnings when using KOMA 
	  with listings package  
o Replaced \mathrm-command with \textrm-command
  (Chapter03.tex)

Changes in version 4.0 (December 2011)
o Due to lots of issues and complaints, 
  classicthesis-preamble.sty is replaced by 
  classicthesis-config.tex (which is cleaner,
  nicer, better, etc. than before!)
o No per-chapter-numbering also for equations 
  (classicthesis.sty and Chapter03.tex)
o classicthesis.sty now also works without the 
  KOMA-classes (scrbook, scrartcl, etc.):
	- This affects the text body shape, where the
	  package "typearea" is always loaded in order 
	  to use \areaset
	- And affects the layout of footnotes where the 
	  package "footmisc" is loaded otherwise
	  (not 100\% identical look-and-feel but OK)
o Help for using spanish babel with classicthesis 
  (classicthesis-config.tex)
o Note about pdfsync issues with graffiti 
  (Chapter01.tex)
o Minor clean-up of comments and duplicate lines 
  (classicthesis.sty)
o Adjusted the colophon text (Colophon.tex)
o Increased space for labels in the LoF, LoT, LoL
o Included version information on the title page and
  in the drafting and final version information 
  (classicthesis.sty and Titlepage.tex)

Changes in version 3.0 (June 2011)
o There have been some major changes in order to port 
  classicthesis to LyX easily. See below for details.
  Special thanks go to Ivo Pletikosi\'c for all his 
  hard work he put into this project!
o Changes in ClassicThesis.tex:
	- Redundant fleqn removed from documentclass options 
	 (will be set by amsmath package in preamble)
	- KOMA adjustments for documentclass: 
	  fontsize=11pt,paper=14
	- Moved language options into documentclass due to LyX
	  issues with babel
o Changes in classicthesis.sty:
	- Removed bcor from \areaset command so that it can
	  be set via \documentclass option (BCOR=)
	- New \ctparttext command for putting preamble text
	  after part titles (see ClassicThesis.tex for examples)
	- \graffito command now also available as original
	  \marginpar (backward compatibility is enabled)
	- Chapter number in margin done with \oldmarginpar
o Changes to classicthesis-preamble.sty:
  - Fixed autoref for subfigures (see Chapter 2 for example)
  - Fixed issues with redefining autoref strings (for
      different languages)
	- Now contains all configuration information, such as
	  the title, your name etc.
	- This package now also loads classicthesis.sty, change
	  the options classicthesis to be loaded with here  
	- Package inputenc now loaded with latin9 option 
	- Package listings now also loaded here
	- Now safer package loading regarding options by
	  using \PassOptionsToPackage command extensively
	- Inserted new string for \mySubtitle
o Changes in Titlepage.tex and Titleback.tex because of new 
  string \mySubtitle
o Changed a lot of the documentation, e.g., in Chapter01.tex

Changes in version 2.9 (January 2011)
o Fixed onlytext euler font for MinionPro font (in 
  classicthesis.sty)
o Option "listsseparated" deprecated, because it led to some
  strange side-effects (in classicthesis.sty)
o Changed default font size to 11pt (in ClassicThesis.tex) and
  adjusted text block size accordingly (in classicthesis.sty)
o Fixed bug with backward compatibility regarding old commands
  \myChapter and \myPart in classicthesis.sty
o New option "floatperchapter" for classicthesis.sty, removed 
  all code for that from classicthesis-ldpkg.sty
o Removed "nochapters" option from classicthesis-ldpkg.sty
o Removed redundant loading of listings package (in
  classicthesis-ldpkg.sty)
o Fixed some headline bug in example classicthesis-book.tex
o Fixed a bug when using parts with plain latex as in example
  classicthesis-book.tex (in classicthesis.sty)

Changes in version 2.8 (March/May 2010)
o Fixed serious \graffito bug in classicthesis.sty
  (thanks to Lorenzo Pantieri and Enrico Gregorio)
o Included backward compatibility regarding old commands
  \myChapter and \myPart in classicthesis.sty
o Fixed drafting issues (draft information not shown at all)
  caused by wrong code for listings and listsseparated options
  in classicthesis.sty 

Changes in version 2.7 (February 2010, cumulative release)
o Removed option for classicthesis-ldpkg.sty: nobackref 
  Introduced instead option "backref" for consistency
  which works the other way (no backrefs by default)
  
Changes in version 2.6.2 (January 2010, released as beta)
o New option for classicthesis-ldpkg.sty: nobackref 
  (removes links to cited page in bibliography)
o Fixed some spacing issues for LoF, LoT, LoL with option
  "listsseparated" (in classicthesis.sty)

Changes in version 2.6.1 (October 2009, released as beta)
o Removed \myChapter and \myPart, you can now use the regular
  \chapter and \part commands (in classicthesis.sty)
  (thanks to Hinrich Harms for this)
o Fixed used KOMA-options: numbers=noenddot, cleardoublepage=empty
  (in ClassicThesis.tex)
o Included hack to use citations in float environments, will 
  be fixed with caption package version 3.2 (in classicthesis.sty)
o Included some font and text area fine-tuning code 
  (in ClassicThesis.tex)
o Some testing with Libertine font (classicthesis-book.tex)
o Fixed numbering of listings used in different chapters
  (in ClassicThesis.tex, classicthesis.sty, classicthesis-ldpkg.sty)
o Spacing between listings in different chapters and after List 
  of Listings header fixed (in classicthesis.sty)
o Increased \newnumberwidth to sizeof(999) which is better for 
  documents with more than 99 pages (in classicthesis.sty)
o New option for classicthesis.sty: manychapters
    
Changes in version 2.6 (August 2009)
o Centered the title page with the addmargin environment
  (thanks to Nicolas Repp for the hint)
o Fixed header for page two of Table of Contents (with 3 
  or more pages) (in Contents.tex)
o Added numbering of \subsubsection (in Contents.tex)
o Added correct Table of Contents entries for \subsubsection
  (in classicthesis.sty)
o Added printonlyused option to loading acronym package
  (in classicthesis-ldpkg.sty)
o Some code for "clean" hyperlinks (w/o color and w/o boxes)
o Minor fix for \graffito (in classicthesis.sty)

Changes in version 2.5.1 (May 2009, released as beta)
o New option for classicthesis.sty: dottedtoc
  (Refer to the manual for more information.)
o New option for classicthesis.sty: listings
  (Refer to the manual for more information.)
  (Credit + thanks to Prof. Enrico Gregorio)
o Minor clean-up and bug-fixing

Changes in version 2.5 (October 2008, cumulative release)
o Increased text-width for better page layout (experimental)
o Cumulative release, some minor clean-up and bug-fixing

Changes in version 2.4.{1--3} (February and April 2008,
released as betas)
o Switched back to "obsolete" KOMA options due to 
  compatibility issues on some installations
o Increased robustness of \cauthor command in 
  classicthesis-ldpk.sty
o Spacing fix for \sectionmark (in classicthesis.sty) 
o Made Booleans private (in classicthesis.sty)
o Acronyms header for long acronym lists (in Contents.tex)
o Moved "amsmath" package from classicthesis.sty to
  ClassicThesis.tex
o "MinionPro" package now loaded with "mathlf" option
  instead of "osf" option (in classicthesis.sty)
o Fixed issue with contents headings (in classicthesis.sty
  and in Contents.tex)
o Thanks to Lorenzo

Changes in version 2.3 (November 2007)
o Fixed serious bug with \myChapter command (using plain 
  LaTeX)
o Removed hypcap package from classicthesis-ldpkg.sty and
  placeins package from classicthesis.sty. Put both into
  ClassicThesis.tex for finer end-user control
o Removed obsolete KOMA options from ClassicThesis.tex
o Option "subfigure" deprecated, replaced by "subfig" (in 
  classicthesis.sty)
o Inserted some mechanisms to detect whether subfig(ure) 
  package was loaded or not (in classicthesis.sty)
o Inserted some mechanism to detect whether classicthesis
  packackage was loaded or not (in classicthesis-ldpkg.sty)
o Moved "headlines" code block a bit up in 
  classicthesis.sty (seemed to cause problems with new
  KOMA-Script classes)
o Removed accidental "natbib" from classicthesis-ldpkg.sty  
o Some fine-tuning in (Dirty)Titlepage.tex
o Thanks to Lorenzo and Denis! :-)

Changes in version 2.2 (October 2007)
o \myChapter and \myPart now take an optional argument
  just as the regular \part and \chapter commands
o Did some minor changes to classicthesis-book.tex
  so it's a better example
o Inserted some \cleardoublepage before \myPart 
  occurences to avoid pdfbookmark problems
o Introduced some general typographic fine-tuning
  (linespread, penalties, etc.)
o Did some fine-tuning of the \graffito command

Changes in version 2.1 (July 2007)
o Removed duplicate xcolor package call from 
  classicthesis-ldpkg.sty and shifed some color
  definitions around
o Removed re-definition of \ttdefault

Changes in version 2.0 (June 2007, cumulative release)
o Better setup of the list of acronyms 
  (in classicthesis-ldpkg.sty)
o Using KOMA option footinclude in ClassicThesis.tex
  (text block sizes are adjusted to this)
o New option for classicthesis.sty: minionpro
o New option for classicthesis.sty: minionprospacing
o New option for classicthesis.sty: pdfspacing
  (Refer to the manual for more information.)

Changes in version 1.7 (May 2007, not released separately)
o Removed \graphicspath from ClassicThesis.tex
o Use the nag package to ensure "compliance"
o Switched from ccaption to caption in classicthesis-ldpkg.sty
  (setup via \captionsetup in ClassicThesis.tex)
o Switched from subfigure to subfig in classicthesis-ldpkg.sty
o Removed obsolete "usenames" option from loading xcolor package
o Noticed problem with \thelstlisting on some installations
  (commented out in classicthesis-ldpkg.sty)
o Noticed problem with some hyperlinks on some installations
  (could not determine cause)

Changes in version 1.6 (April 2007, not released separately)
o Included greetings to Lorenzo Pantieri for many very useful
  suggestions
o Introduced new commands in classicthesis-ldpkg.sty to make
  adaptation of backrefs to different languages easier
   - \backrefnotcitedstring (ref is not cited)
   - \backrefcitedsinglestring (ref is cited on one page)
   - \backrefcitedmultistring (ref is cited on multiple pages)
o Removed ellipsis package from classicthesis-ldpkg.sty due to 
  some undesired results for some users
o Removed the following packages from classicthesis-ldpkg.sty as 
  these seem to require changes to their options from most users:
  inputenc, babel, natbib (now in ClassicThesis.tex)
o New option for classicthesis-ldpkg.sty: nochapters
  Use the package with classes that do not have chapter divisions 

Changes in version 1.5 (April 2007, not released separately)
o Fixed some bugs to use classicthesis.sty for article layout
o Inserted some info/warnings when using nochapter/parts
o Extended the manual: examples for using classicthesis.sty for
  other projects than a thesis (source available in folder
  "Examples")
o Some minor adjustments in classicthesis-ldpkg.sty
o Fixed some spelling mistakes

Changes in version 1.4.2 (March 2007)
o Renamed loadpackages.sty to classicthesis-ldpkg.sty due to
  TeX Live package tree issues

Changes in version 1.4.1 (March 2007)
o Fixed some wording concerning the license :-o
o Added fixltx2e and ellipsis packages to to loadpackages.sty to correct
  some minor glitches
o Fixed and changed some things about ToC entries of parts
o Some minor bug fixes

Changes in version 1.4 (January 2007)
o Replaced \lineheight with \baselineskip in classicthesis.sty
o Removed obsolete "usenames" option from xcolor package (classicthesis.sty)
o Now classicthesis.sty processes the global a5paper option and adjusts 
  the layout accordingly (experimental!)

Changes in version 1.3.1 (August 2006)
o Urgent bug concerning ToC spacing etc. fixed

Changes in version 1.3 (August 2006) 
o New option for classicthesis.sty: parts
  Turn this on if you use Part divisions. It fine-tunes the ToC and
  adds support for Part division via \myPart{} (cf. \myChapter{})
  (The style of this feature is preliminary, any suggestions?!)
o New option for classicthesis.sty: eulermath
  Uses the awesome Euler fonts for math (Palatino fonts are default).
o Added mparhack package to loadpackages.sty to get the graffiti right
o Added a hint to loadpackages.sty on how to typeset the List of 
  Listings consistently with classicthesis
o Some minor fine-tuning of typographic details
o Collaboration with babel package improved (now easier to use
  with other languages than English)
o Added appropriate textwidth values for 11pt Palatino and Minion
  (See comments near \areaset in classicthesis.sty)
o Note: There is a problem with the case of math text in part-, 
  chapter-, and section titles and I have no clue how to fix this 
  (either the case or the spacing breaks). So far, I chose the case. :-(

Changes in version 1.2 (June 2006)
o Setup a little postcard collection: http://postcards.miede.de
o Changed stupid spelling mistake: "A Homage" => "An Homage" D'oh!
o New option for classicthesis.sty: nochapters
  Allows to use the look-and-feel with classes that do not use chapters.
o New option for classicthesis.sty: beramono
  Loads Bera Mono as typewriter font. (Default = no typewriter font.)
o Included list of files, see LISTOFFILES.  

Changes in version 1.1 (May 2006)
o classicthesis.sty now stand-alone and usable w/o whole bundle!
o classicthesis.sty compatible with both LaTeX and PDFLaTeX
  Note: this is only true for classicthesis.sty, not the whole bundle.
o New option for classicthesis.sty: subfigure
  Tells the style to add the respective option when loading tocloft.
o Now loading microtype package w/o options (classicthesis.sty)
o Fixed overfull hbox warnings for ToC entries (classicthesis.sty)
o No longer depending on a particular caption package (classicthesis.sty)
o Layout for subsubsections provided (classicthesis.sty)
o PDF opens on title page (ClassicThesis.[tex|pdf])
o Files are a bit more "ASCII-friendly" (all)
o Note: Thanks to all the folks who already sent me a postcard! :-)

Version 1.0 (March 2006)
o First public release

==> template/classicthesis-config.tex <==
% ****************************************************************************************************
% classicthesis-config.tex 
% formerly known as loadpackages.sty, classicthesis-ldpkg.sty, and classicthesis-preamble.sty 
% Use it at the beginning of your ClassicThesis.tex, or as a LaTeX Preamble 
% in your ClassicThesis.{tex,lyx} with \input{classicthesis-config}
% ****************************************************************************************************  
% If you like the classicthesis, then I would appreciate a postcard. 
% My address can be found in the file ClassicThesis.pdf. A collection 
% of the postcards I received so far is available online at 
% http://postcards.miede.de
% ****************************************************************************************************


% ****************************************************************************************************
% 0. Set the encoding of your files. UTF-8 is the only sensible encoding nowadays. If you can't read
% äöüßáéçèê∂åëæƒÏ€ then change the encoding setting in your editor, not the line below. If your editor
% does not support utf8 use another editor!
% ****************************************************************************************************
\PassOptionsToPackage{utf8}{inputenc}
	\usepackage{inputenc}

% ****************************************************************************************************
% 1. Configure classicthesis for your needs here, e.g., remove "drafting" below 
% in order to deactivate the time-stamp on the pages
% ****************************************************************************************************
\PassOptionsToPackage{eulerchapternumbers,listings,drafting,%
					 pdfspacing,%floatperchapter,%linedheaders,%
					 subfig,beramono,eulermath,parts}{classicthesis}                                        
% ********************************************************************
% Available options for classicthesis.sty 
% (see ClassicThesis.pdf for more information):
% drafting
% parts nochapters linedheaders
% eulerchapternumbers beramono eulermath pdfspacing minionprospacing
% tocaligned dottedtoc manychapters
% listings floatperchapter subfig
% ********************************************************************


% ****************************************************************************************************
% 2. Personal data and user ad-hoc commands
% ****************************************************************************************************
\newcommand{\myTitle}{A Classic Thesis Style\xspace}
\newcommand{\mySubtitle}{An Homage to The Elements of Typographic Style\xspace}
\newcommand{\myDegree}{Doktor-Ingenieur (Dr.-Ing.)\xspace}
\newcommand{\myName}{André Miede\xspace}
\newcommand{\myProf}{Put name here\xspace}
\newcommand{\myOtherProf}{Put name here\xspace}
\newcommand{\mySupervisor}{Put name here\xspace}
\newcommand{\myFaculty}{Put data here\xspace}
\newcommand{\myDepartment}{Put data here\xspace}
\newcommand{\myUni}{Put data here\xspace}
\newcommand{\myLocation}{Saarbrücken\xspace}
\newcommand{\myTime}{September 2015\xspace}
\newcommand{\myVersion}{version 4.2\xspace}

% ********************************************************************
% Setup, finetuning, and useful commands
% ********************************************************************
\newcounter{dummy} % necessary for correct hyperlinks (to index, bib, etc.)
\newlength{\abcd} % for ab..z string length calculation
\providecommand{\mLyX}{L\kern-.1667em\lower.25em\hbox{Y}\kern-.125emX\@}
\newcommand{\ie}{i.\,e.}
\newcommand{\Ie}{I.\,e.}
\newcommand{\eg}{e.\,g.}
\newcommand{\Eg}{E.\,g.} 
% ****************************************************************************************************


% ****************************************************************************************************
% 3. Loading some handy packages
% ****************************************************************************************************
% ******************************************************************** 
% Packages with options that might require adjustments
% ******************************************************************** 
%\PassOptionsToPackage{ngerman,american}{babel}   % change this to your language(s)
% Spanish languages need extra options in order to work with this template
%\PassOptionsToPackage{spanish,es-lcroman}{babel}
	\usepackage{babel}                  

\usepackage{csquotes}
\PassOptionsToPackage{%
    %backend=biber, %instead of bibtex
	backend=bibtex8,bibencoding=ascii,%
	language=auto,%
	style=numeric-comp,%
    %style=authoryear-comp, % Author 1999, 2010
    %bibstyle=authoryear,dashed=false, % dashed: substitute rep. author with ---
    sorting=nyt, % name, year, title
    maxbibnames=10, % default: 3, et al.
    %backref=true,%
    natbib=true % natbib compatibility mode (\citep and \citet still work)
}{biblatex}
    \usepackage{biblatex}

\PassOptionsToPackage{fleqn}{amsmath}       % math environments and more by the AMS 
    \usepackage{amsmath}

% ******************************************************************** 
% General useful packages
% ******************************************************************** 
\PassOptionsToPackage{T1}{fontenc} % T2A for cyrillics
    \usepackage{fontenc}     
\usepackage{textcomp} % fix warning with missing font shapes
\usepackage{scrhack} % fix warnings when using KOMA with listings package          
\usepackage{xspace} % to get the spacing after macros right  
\usepackage{mparhack} % get marginpar right
\usepackage{fixltx2e} % fixes some LaTeX stuff --> since 2015 in the LaTeX kernel (see below)
%\usepackage[latest]{latexrelease} % will be used once available in more distributions (ISSUE #107)
\PassOptionsToPackage{printonlyused,smaller}{acronym} 
    \usepackage{acronym} % nice macros for handling all acronyms in the thesis
    %\renewcommand{\bflabel}[1]{{#1}\hfill} % fix the list of acronyms --> no longer working
    %\renewcommand*{\acsfont}[1]{\textsc{#1}} 
    \renewcommand*{\aclabelfont}[1]{\acsfont{#1}}
% ****************************************************************************************************


% ****************************************************************************************************
% 4. Setup floats: tables, (sub)figures, and captions
% ****************************************************************************************************
\usepackage{tabularx} % better tables
    \setlength{\extrarowheight}{3pt} % increase table row height
\newcommand{\tableheadline}[1]{\multicolumn{1}{c}{\spacedlowsmallcaps{#1}}}
\newcommand{\myfloatalign}{\centering} % to be used with each float for alignment
\usepackage{caption}
% Thanks to cgnieder and Claus Lahiri
% http://tex.stackexchange.com/questions/69349/spacedlowsmallcaps-in-caption-label
% [REMOVED DUE TO OTHER PROBLEMS, SEE ISSUE #82]    
%\DeclareCaptionLabelFormat{smallcaps}{\bothIfFirst{#1}{~}\MakeTextLowercase{\textsc{#2}}}
%\captionsetup{font=small,labelformat=smallcaps} % format=hang,
\captionsetup{font=small} % format=hang,
\usepackage{subfig}  
% ****************************************************************************************************


% ****************************************************************************************************
% 5. Setup code listings
% ****************************************************************************************************
\usepackage{listings} 
%\lstset{emph={trueIndex,root},emphstyle=\color{BlueViolet}}%\underbar} % for special keywords
\lstset{language=[LaTeX]Tex,%C++,
    morekeywords={PassOptionsToPackage,selectlanguage},
    keywordstyle=\color{RoyalBlue},%\bfseries,
    basicstyle=\small\ttfamily,
    %identifierstyle=\color{NavyBlue},
    commentstyle=\color{Green}\ttfamily,
    stringstyle=\rmfamily,
    numbers=none,%left,%
    numberstyle=\scriptsize,%\tiny
    stepnumber=5,
    numbersep=8pt,
    showstringspaces=false,
    breaklines=true,
    %frameround=ftff,
    %frame=single,
    belowcaptionskip=.75\baselineskip
    %frame=L
} 
% ****************************************************************************************************             


% ****************************************************************************************************
% 6. PDFLaTeX, hyperreferences and citation backreferences
% ****************************************************************************************************
% ********************************************************************
% Using PDFLaTeX
% ********************************************************************
\PassOptionsToPackage{pdftex,hyperfootnotes=false,pdfpagelabels}{hyperref}
    \usepackage{hyperref}  % backref linktocpage pagebackref
\pdfcompresslevel=9
\pdfadjustspacing=1 
\PassOptionsToPackage{pdftex}{graphicx}
    \usepackage{graphicx} 
 

% ********************************************************************
% Hyperreferences
% ********************************************************************
\hypersetup{%
    %draft, % = no hyperlinking at all (useful in b/w printouts)
    colorlinks=true, linktocpage=true, pdfstartpage=3, pdfstartview=FitV,%
    % uncomment the following line if you want to have black links (e.g., for printing)
    %colorlinks=false, linktocpage=false, pdfstartpage=3, pdfstartview=FitV, pdfborder={0 0 0},%
    breaklinks=true, pdfpagemode=UseNone, pageanchor=true, pdfpagemode=UseOutlines,%
    plainpages=false, bookmarksnumbered, bookmarksopen=true, bookmarksopenlevel=1,%
    hypertexnames=true, pdfhighlight=/O,%nesting=true,%frenchlinks,%
    urlcolor=webbrown, linkcolor=RoyalBlue, citecolor=webgreen, %pagecolor=RoyalBlue,%
    %urlcolor=Black, linkcolor=Black, citecolor=Black, %pagecolor=Black,%
    pdftitle={\myTitle},%
    pdfauthor={\textcopyright\ \myName, \myUni, \myFaculty},%
    pdfsubject={},%
    pdfkeywords={},%
    pdfcreator={pdfLaTeX},%
    pdfproducer={LaTeX with hyperref and classicthesis}%
}   

% ********************************************************************
% Setup autoreferences
% ********************************************************************
% There are some issues regarding autorefnames
% http://www.ureader.de/msg/136221647.aspx
% http://www.tex.ac.uk/cgi-bin/texfaq2html?label=latexwords
% you have to redefine the makros for the 
% language you use, e.g., american, ngerman
% (as chosen when loading babel/AtBeginDocument)
% ********************************************************************
\makeatletter
\@ifpackageloaded{babel}%
    {%
       \addto\extrasamerican{%
			\renewcommand*{\figureautorefname}{Figure}%
			\renewcommand*{\tableautorefname}{Table}%
			\renewcommand*{\partautorefname}{Part}%
			\renewcommand*{\chapterautorefname}{Chapter}%
			\renewcommand*{\sectionautorefname}{Section}%
			\renewcommand*{\subsectionautorefname}{Section}%
			\renewcommand*{\subsubsectionautorefname}{Section}%     
                }%
       \addto\extrasngerman{% 
			\renewcommand*{\paragraphautorefname}{Absatz}%
			\renewcommand*{\subparagraphautorefname}{Unterabsatz}%
			\renewcommand*{\footnoteautorefname}{Fu\"snote}%
			\renewcommand*{\FancyVerbLineautorefname}{Zeile}%
			\renewcommand*{\theoremautorefname}{Theorem}%
			\renewcommand*{\appendixautorefname}{Anhang}%
			\renewcommand*{\equationautorefname}{Gleichung}%        
			\renewcommand*{\itemautorefname}{Punkt}%
                }%  
            % Fix to getting autorefs for subfigures right (thanks to Belinda Vogt for changing the definition)
            \providecommand{\subfigureautorefname}{\figureautorefname}%             
    }{\relax}
\makeatother


% ****************************************************************************************************
% 7. Last calls before the bar closes
% ****************************************************************************************************
% ********************************************************************
% Development Stuff
% ********************************************************************
\listfiles
%\PassOptionsToPackage{l2tabu,orthodox,abort}{nag}
%   \usepackage{nag}
%\PassOptionsToPackage{warning, all}{onlyamsmath}
%   \usepackage{onlyamsmath}

% ********************************************************************
% Last, but not least...
% ********************************************************************
\usepackage{classicthesis} 
% ****************************************************************************************************


% ****************************************************************************************************
% 8. Further adjustments (experimental)
% ****************************************************************************************************
% ********************************************************************
% Changing the text area
% ********************************************************************
%\linespread{1.05} % a bit more for Palatino
%\areaset[current]{312pt}{761pt} % 686 (factor 2.2) + 33 head + 42 head \the\footskip
%\setlength{\marginparwidth}{7em}%
%\setlength{\marginparsep}{2em}%

% ********************************************************************
% Using different fonts
% ********************************************************************
%\usepackage[oldstylenums]{kpfonts} % oldstyle notextcomp
%\usepackage[osf]{libertine}
%\usepackage[light,condensed,math]{iwona}
%\renewcommand{\sfdefault}{iwona}
%\usepackage{lmodern} % <-- no osf support :-(
%\usepackage{cfr-lm} % 
%\usepackage[urw-garamond]{mathdesign} <-- no osf support :-(
%\usepackage[default,osfigures]{opensans} % scale=0.95 
%\usepackage[sfdefault]{FiraSans}
% ****************************************************************************************************

